On the connection between the intergalactic medium and galaxies: The HI-galaxy cross-correlation at z < 1

We present a new optical spectroscopic survey of 1777 'star-forming' ('SF') and 366 'non-star-forming' ('non-SF') galaxies at redshifts z < 1 (2143 in total), 22 AGN and 423 stars, observed by instruments such as DEIMOS, VIMOS and GMOS, in 3 fields containing 5 quasi-stellar objects (QSOs) with HST UV spectroscopy. We also present a new spectroscopic survey of 165 'strong' (10^14 < NHI < 10^17 cm^-2), and 489 'weak' (10^13 < NHI < 10^14 cm^-2) intervening HI absorption line systems at z < 1 (654 in total), observed in the spectra of 8 QSOs by COS and FOS on the HST. Combining these new data with previously published galaxy catalogs such as VVDS and GDDS, we have gathered a sample of 654 HI absorption systems and 17509 galaxies at transverse scales < 50 Mpc. We present observational results on the HI-galaxy and galaxy-galaxy correlations at transverse scales r < 10 Mpc, and the HI-HI auto-correlation at transverse scales r < 2 Mpc. The two-point correlation functions are measured both along and transverse to the line-of-sight. We constrain the HI-galaxy statistical connection, as a function of both HI column density and galaxy star-forming activity. Our results are consistent with the following conclusions: (1) the bulk of HI systems on Mpc scales have little velocity dispersion (<120 km/s) with respect to the bulk of galaxies; (2) the vast majority of strong HI systems and SF galaxies are distributed in the same locations, together with 75+-15% of non-SF galaxies, all of which typically reside in dark matter haloes of similar masses; (3) 25+-15% of non-SF galaxies reside in galaxy clusters and are not correlated with strong HI systems at scales < 2 Mpc; and (4) 50% of weak HI systems reside within galaxy voids (hence not correlated with galaxies), and are confined in dark matter haloes of masses smaller than those hosting... [abridged]

==> figs/Q0107_completeness_DEIMOS_input.tex <==
\begin{figure*}
  \begin{minipage}{0.49\textwidth}
  \includegraphics[width=1.05\textwidth]{/home/ntejos/abs-gal/figs/Q0107_completeness_DEIMOS_1.eps}
  \end{minipage}
  \begin{minipage}{0.49\textwidth}
  \includegraphics[width=1.05\textwidth]{/home/ntejos/abs-gal/figs/Q0107_completeness_DEIMOS_2.eps}
  \end{minipage}
    
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Same as Figure \ref{fig:VIMOS_completeness} but for DEIMOS
    observation of Q0107 field.}\label{fig:Q0107_completeness_DEIMOS}

\end{figure*}


==> figs/Q0107_completeness_GMOS_input.tex <==
\begin{figure*}
  \begin{minipage}{0.49\textwidth}
  \includegraphics[width=1.05\textwidth]{/home/ntejos/abs-gal/figs/Q0107_completeness_GMOS_1.eps}
  \end{minipage}
  \begin{minipage}{0.49\textwidth}
  \includegraphics[width=1.05\textwidth]{/home/ntejos/abs-gal/figs/Q0107_completeness_GMOS_2.eps}
  \end{minipage}
    
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Same as Figure \ref{fig:VIMOS_completeness} but for GMOS
    observation of Q0107 field.}\label{fig:Q0107_completeness_GMOS}

\end{figure*}


==> figs/Q0107_completeness_VIMOS_input.tex <==
\begin{figure*}
  \begin{minipage}{0.49\textwidth}
  \includegraphics[width=1.05\textwidth]{/home/ntejos/abs-gal/figs/Q0107_completeness_VIMOS_1.eps}
  \end{minipage}
  \begin{minipage}{0.49\textwidth}
  \includegraphics[width=1.05\textwidth]{/home/ntejos/abs-gal/figs/Q0107_completeness_VIMOS_2.eps}
  \end{minipage}
    
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Same as Figure \ref{fig:VIMOS_completeness} but for VIMOS
    observation of Q0107 field.}\label{fig:Q0107_completeness_VIMOS}

\end{figure*}


==> figs/VIMOS_completeness_1_input.tex <==
\begin{figure*}
  \includegraphics[width=1.0\textwidth]{/home/ntejos/abs-gal/figs/VIMOS_completeness_1.eps}
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Completeness of our VIMOS survey for fields J1005, J1022 and
    J2218. The panels show the fraction of targeted objects with
    assigned redshift (left panel); the fraction of targeted objects
    with redshift that were identified as galaxies (middle panel); and
    the fraction of targeted objects with redshift that were identified
    as stars (right panel); all of which as function of apparent
    \rband~magnitude. These fractions are shown for both objects with
    redshifts labeled as `a' (`secure', solid green lines) and as `a+b'
    (`secure+possible', dashed red lines). The number of objects
    corresponding to a fraction of $1$ (total) are labeled at the
    bottom of each magnitude bin.}

  \label{fig:VIMOS_completeness_1}
\end{figure*}


==> figs/VIMOS_completeness_2_input.tex <==
\begin{figure*}
  \includegraphics[width=0.7\textwidth]{/home/ntejos/abs-gal/figs/VIMOS_completeness_2.eps}
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Fraction of `emission' (blue lines) and/or `absorption' (red
    lines) galaxies with respect to the total number of galaxies
    detected in our VIMOS survey in fields J1005, J1022 and J2218, as a
    function of \rband~magnitude (left panel) and redshift (right
    panel). These fractions are shown for both galaxies with redshifts
    labeled as `a' (`secure', solid lines) and as `a+b'
    (`secure+possible', dashed lines). The number of objects
    corresponding to a fraction of $1$ (total) are labeled at the
    bottom of each magnitude and redshift bin.}

  \label{fig:VIMOS_completeness_2}
\end{figure*}


==> figs/VIMOS_completeness_input.tex <==
\begin{figure*}
  \begin{minipage}{0.49\textwidth}
  \includegraphics[width=1.05\textwidth]{/home/ntejos/abs-gal/figs/VIMOS_completeness_VIMOS_1.eps}
  \end{minipage}
  \begin{minipage}{0.49\textwidth}
  \includegraphics[width=1.05\textwidth]{/home/ntejos/abs-gal/figs/VIMOS_completeness_VIMOS_2.eps}
  \end{minipage}
    
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Completeness of our VIMOS survey for fields J1005, J1022 and
    J2218. The first and second panels show the fraction of targeted
    objects with assigned redshift and the fraction of those that were
    identified as galaxies (black lines) and/or stars (yellow lines),
    as function of apparent \rband~magnitude, respectively. The third
    and fourth panels show the fraction of galaxies that were
    classified as `star-forming' (blue lines) and/or `non-star-forming'
    (red lines), as a function of \rband~magnitude and redshift,
    respectively. All these fractions are shown for both objects with
    high (`a' label; solid lines) and/or any (`a+b' label; dashed
    lines) confidence redshifts. The number of objects corresponding to
    a fraction of $1$ (total) are labeled at the bottom of each
    bin.}\label{fig:VIMOS_completeness}

\end{figure*}


==> figs/all_xi_input.tex <==
\begin{figure*}
  \begin{minipage}{1.05\textwidth}
    \centering
    \includegraphics[height=6.5cm]{/home/ntejos/abs-gal/figs/all_xi.eps}
  \end{minipage}
    %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Total number of cross-pairs between \hi~absorption systems
    and galaxies as a function of separations along ($\pi$; $y$-axes)
    and transverse to the line-of-sight ($\sigma$; $x$-axes). We used
    an arbitrary binning of $0.5$ \mpc~with a Gaussian smoothing of
    standard deviation of $0.5$ \mpc~along both
    directions.} \label{fig:counts_ag}

\end{figure*}



==> figs/counts_gg_input.tex <==
\begin{figure*}
  \includegraphics[height=6.5cm]{/home/ntejos/abs-gal/figs/counts_gg.eps}
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Total number of galaxy pairs as a function of separations
    along the line-of-sight ($\pi$; $y$-axes) and separations
    transverse to the line-of-sight ($\sigma$; $x$-axes). We used an
    arbitrary binning of $XX$ \mpc~along both directions and we have
    truncated the axes at arbitrary distances. From left to right we
    have $D_{\rm g}D_{\rm g}$, $D_{\rm g}R_{\rm g}$, and $R_{\rm
      g}R_{\rm g}$.} \label{fig:counts_gg}

\end{figure*}



==> figs/counts_input.tex <==
\begin{figure*}
  \begin{minipage}{1.05\textwidth}
    \centering
    \includegraphics[height=6.5cm]{/home/ntejos/abs-gal/figs/counts_ag.eps}
  \end{minipage}
  \begin{minipage}{1.05\textwidth}
    \centering
    \includegraphics[height=6.5cm]{/home/ntejos/abs-gal/figs/counts_gg.eps}
  \end{minipage}
  \begin{minipage}{1.05\textwidth}
    \centering
    \includegraphics[height=6.5cm]{/home/ntejos/abs-gal/figs/counts_aa.eps}
  \end{minipage}
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Total number of cross-pairs between \hi~absorption systems
    and galaxies (top panels), galaxies and galaxies (middle panels)
    and \hi-\hi~absorption systems (bottom panels), as a function of
    separations along ($\pi$; $y$-axes) and transverse to the
    line-of-sight ($\sigma$; $x$-axes). We used an arbitrary binning of
    $0.5$ \mpc~with a Gaussian smoothing of standard deviation of $0.5$
    \mpc~along both directions.} \label{fig:counts}

\end{figure*}


==> figs/errors_ag_input.tex <==
\begin{figure*}
  \begin{minipage}{\textwidth}
    \flushleft
  \includegraphics[width=\textwidth]{/home/ntejos/abs-gal/figs/errors_ag.eps}
  \end{minipage}

  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Uncertainty estimations (squared root of variances) of the
    observed \hi-galaxy cross-correlation, $\xi^{\rm LS}_{\rm ag}$, for
    our full sample as a function of separations along the
    line-of-sight ($\pi$; $y$-axes) and separations transverse to the
    line-of-sight ($\sigma$; $x$-axes). We used an arbitrary binning of
    $1$ \mpc~along both directions and we have truncated the axes at
    arbitrary distances. From left to right: uncertainty from the
    \citet{landy93} analytical approximation, $\Delta_{\rm LS}$
    (equation \ref{eq:var_LS}); uncertainty from a `jacknife'
    resampling technique, $\Delta_{\rm JK}$ (equation \ref{eq:var_JK});
    uncertainty from a `bootstrap' resampling technique, $\Delta_{\rm
      BS}$ (equation \ref{eq:var_BS}); and the absolute difference
    between $\Delta_{\rm LS}$ and $\Delta_{\rm BS}$. Both $\Delta_{\rm
      LS}$ and $\Delta_{\rm BS}$ are found to be very similar while
    $\Delta_{\rm JK}$ might be overestimating the true
    uncertainty} \label{fig:errors_ag}

\end{figure*}



==> figs/errors_gg_input.tex <==
\begin{figure*}
  \includegraphics[height=6.5cm]{/home/ntejos/abs-gal/figs/errors_gg.eps}
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Uncertainty estimations (squared root of variances) of the
    observed galaxy auto-correlation, $\xi^{\rm LS}_{\rm gg}$, for our
    full sample as a function of separations along the line-of-sight
    ($\pi$; $y$-axes) and separations transverse to the line-of-sight
    ($\sigma$; $x$-axes). We used an arbitrary binning of $1$
    \mpc~along both directions and we have truncated the axes at
    arbitrary distances. From left to right: uncertainty from the
    \citet{landy93} analytical approximation, $\Delta_{\rm LS}$
    (equation \ref{eq:var_LS}); uncertainty from a `jacknife'
    resampling technique, $\Delta_{\rm JK}$ (equation \ref{eq:var_JK});
    uncertainty from a `bootstrap' resampling technique, $\Delta_{\rm
      BS}$ (equation \ref{eq:var_BS}); and the absolute difference
    between $\Delta_{\rm LS}$ and $\Delta_{\rm BS}$. Both $\Delta_{\rm
      LS}$ and $\Delta_{\rm BS}$ are found to be very similar while
    $\Delta_{\rm JK}$ might be overestimating the true
    uncertainty.} \label{fig:errors_gg}

\end{figure*}



==> figs/logn_lims_input.tex <==
\begin{figure}
  \includegraphics[width=0.45\textwidth]{figs/logn_limits.pdf}
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Uncertainty estimations (square root of variances) of the
    projected \hi-galaxy cross-correlation ($\Xi_{\rm ag}$; squares)
    and galaxy auto-correlation ($\Xi_{\rm gg}$; circles) measured from
    our full sample as a function of separations transverse to the
    line-of-sight ($r_{\perp}$). The top panel shows the uncertainty
    from the \citet{Landy1993} analytical approximation, $\Delta_{\rm
      LS}$ (\Cref{eq:var_LS}; green lines); uncertainty from a
    `jackknife' resampling, $\Delta_{\rm JK}$ (\Cref{eq:var_JK}; red
    lines); uncertainty from a `bootstrap' resampling, $\Delta_{\rm
      BS}$ (\Cref{eq:var_BS}; blue lines); and the commonly used
    Poissonian uncertainty, $\Delta_{\rm DD}$ (\Cref{eq:var_DD}; yellow
    lines). The bottom panel shows the ratio between these
    uncertainties and $\Delta_{\rm BS}$.}\label{fig:errors_T}

\end{figure}



==> figs/yz_hist_input.tex <==
\begin{figure*}
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=1\textwidth]{/home/ntejos/abs-gal/figs/zhist_gal_Q0107.pdf}
  \end{minipage}
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=1\textwidth]{/home/ntejos/abs-gal/figs/zhist_gal_J0209.pdf}
  \end{minipage}
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=1\textwidth]{/home/ntejos/abs-gal/figs/zhist_gal_J1005.pdf}
  \end{minipage}
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=1\textwidth]{/home/ntejos/abs-gal/figs/zhist_gal_J1022.pdf}
  \end{minipage}
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=1\textwidth]{/home/ntejos/abs-gal/figs/zhist_gal_J1357.pdf}
  \end{minipage}
  \begin{minipage}{0.49\textwidth}
    \includegraphics[width=1\textwidth]{/home/ntejos/abs-gal/figs/zhist_gal_J2218.pdf}
  \end{minipage}
    
  %% to include a figure, or
  %%\vspace{3.5cm}
  %% to leave a blank space
  \caption{Histograms of the galaxy redshift distribution for our
    different fields ($0.02$ bining).  The black thick solid lines
    correspond to the real distributions whereas the red thin solid
    lines correspond to the normalized random expectation drawn from
    samples of $10 \times$ the real sample sizes. A full description of
    the random generator algorithm can be found in
    \Cref{random:gal}. Top panels show the full galaxy samples while
    the middle and bottom panels show subsamples based on
    \rband~magnitude cuts.}\label{fig:zhist_gal}

\end{figure*}


==> tabs/HI.tex <==
\begin{table*}
  \centering
  %\begin{minipage}{180mm}
    \caption{Properties of the observed QSOs.}\label{tab:data:IGM}
    \begin{tabular}{@{}lcclcccc@{}}
      \hline
      
      QSO Name & Field Name & R.A. (J2000)  & Dec. (J2000) & $z_{\rm QSO}$ & \multicolumn{3}{c}{Magnitude}\\
               &               &              &            &              & Visual (Band) & NUV\tablenotemark{a} & FUV\tablenotemark{a}\\ 
      \hline
 
      
      Q0107-025A           &Q0107& 01 10 13.10   &  $-$02 19 52.0 & 0.96000 & 18.1 ($B$)& XX & YY \\
      Q0107-025B           &Q0107& 01 10 16.20   &  $-$02 18 50.0 & 0.95600 & 17.4 ($V$)& XX & YY \\
      Q0107-0232           &Q0107& 01 10 14.51   &  $-$02 16 57.5 & 0.72600 & 18.4 ($B$)& XX & YY \\
      J020930.7-043826     &J0209& 02 09 30.74   &  $-$04 38 26.3 & 1.12800 & 17.2 ($g$)& XX & XX \\
      J100535.24+013445.7  &J1005& 10 05 35.26   &  $+$01 34 45.6 & 1.08090 & 16.8 ($g$)& XX & XX \\ 
      J102218.99+013218.8  &J1022& 10 22 18.99   &  $+$01 32 18.8 & 0.78900 &           &    &    \\   
      J135726.27+043541.4  &J1357& 13 57 26.27   &  $+$04 35 41.4 & 1.23176 & 17.2 ($g$)& XX & XX \\
      J221806.67+005223.6  &J1022& 22 18 06.69   &  $+$00 52 23.7 & 1.27327 & 17.8 ($V$)& XX & XX \\

      \hline

    \end{tabular}
    \tablenotetext{a}{From GALEX filters.}
    
  %\end{minipage}
\end{table*}


==> tabs/HI_J1005_body.tex <==

\begin{table*}
\centering
\begin{minipage}{\textwidth}
\caption{\hi~absorption systems in QSO J100535.24+013445.7.}\label{tab:HI_J1005}
\begin{tabular}{@{}cc.ccc.@{}}

\hline                            

$z$ & $\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) & & $z&
$\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) \ 


\hline
0.00428 $\pm$ 0.00011 & 14.55 $\pm$ 1.30 & 46 $\pm$ 30 & & 0.23473 $\pm$ 0.00005 & 12.70 $\pm$ 0.28 & 8 $\pm$ 29 \\ 
0.00600 $\pm$ 0.00004 & 13.01 $\pm$ 0.14 & 31 $\pm$ 17 & & 0.24757 $\pm$ 0.00001 & 13.69 $\pm$ 0.03 & 36 $\pm$ 4 \\ 
0.01767 $\pm$ 0.00002 & 13.21 $\pm$ 0.09 & 25 $\pm$ 10 & & 0.25360 $\pm$ 0.00007 & 12.58 $\pm$ 0.50 & 10 $\pm$ 31 \\ 
0.01872 $\pm$ 0.00001 & 13.53 $\pm$ 0.45 & 8 $\pm$ 6 & & 0.25374 $\pm$ 0.00002 & 13.22 $\pm$ 0.12 & 13 $\pm$ 9 \\ 
0.02095 $\pm$ 0.00002 & 13.23 $\pm$ 0.08 & 29 $\pm$ 10 & & 0.25998 $\pm$ 0.00004 & 12.40 $\pm$ 0.26 & 9 $\pm$ 24 \\ 
0.02390 $\pm$ 0.00005 & 13.19 $\pm$ 0.24 & 28 $\pm$ 22 & & 0.26034 $\pm$ 0.00004 & 13.19 $\pm$ 0.26 & 25 $\pm$ 11 \\ 
0.02416 $\pm$ 0.00001 & 14.30 $\pm$ 0.15 & 27 $\pm$ 9 & & 0.26061 $\pm$ 0.00013 & 13.04 $\pm$ 0.42 & 45 $\pm$ 48 \\ 
0.02435 $\pm$ 0.00003 & 13.23 $\pm$ 0.29 & 8 $\pm$ 14 & & 0.26096 $\pm$ 0.00002 & 12.86 $\pm$ 0.14 & 8 $\pm$ 11 \\ 
0.02542 $\pm$ 0.00002 & 13.10 $\pm$ 0.09 & 19 $\pm$ 9 & & 0.26125 $\pm$ 0.00001 & 13.05 $\pm$ 0.14 & 8 $\pm$ 7 \\ 
0.03021 $\pm$ 0.00001 & 13.17 $\pm$ 0.22 & 8 $\pm$ 9 & & 0.26345 $\pm$ 0.00008 & 13.02 $\pm$ 0.87 & 8 $\pm$ 20 \\ 
0.03073 $\pm$ 0.00001 & 13.75 $\pm$ 0.05 & 35 $\pm$ 6 & & 0.26358 $\pm$ 0.00005 & 13.68 $\pm$ 0.66 & 16 $\pm$ 28 \\ 
0.03118 $\pm$ 0.00006 & 13.09 $\pm$ 0.23 & 32 $\pm$ 31 & & 0.26379 $\pm$ 0.00027 & 14.35 $\pm$ 3.83 & 25 $\pm$ 46 \\ 
0.03217 $\pm$ 0.00001 & 13.77 $\pm$ 0.07 & 18 $\pm$ 5 & & 0.26967 $\pm$ 0.00005 & 12.86 $\pm$ 0.27 & 8 $\pm$ 20 \\ 
0.03236 $\pm$ 0.00001 & 14.22 $\pm$ 0.21 & 20 $\pm$ 5 & & 0.26979 $\pm$ 0.00007 & 12.58 $\pm$ 0.65 & 8 $\pm$ 48 \\ 
0.03640 $\pm$ 0.00003 & 13.43 $\pm$ 0.12 & 35 $\pm$ 14 & & 0.26994 $\pm$ 0.00001 & 13.30 $\pm$ 0.11 & 9 $\pm$ 6 \\ 
0.04124 $\pm$ 0.00001 & 13.88 $\pm$ 0.03 & 48 $\pm$ 4 & & 0.27708 $\pm$ 0.00001 & 13.66 $\pm$ 0.03 & 36 $\pm$ 3 \\ 
0.04291 $\pm$ 0.00003 & 13.42 $\pm$ 0.07 & 60 $\pm$ 14 & & 0.27894 $\pm$ 0.00002 & 12.99 $\pm$ 0.09 & 18 $\pm$ 8 \\ 
0.04483 $\pm$ 0.00001 & 13.70 $\pm$ 0.04 & 38 $\pm$ 5 & & 0.28353 $\pm$ 0.00001 & 13.03 $\pm$ 0.08 & 11 $\pm$ 6 \\ 
0.04597 $\pm$ 0.00003 & 13.53 $\pm$ 0.06 & 63 $\pm$ 12 & & 0.29806 $\pm$ 0.00001 & 13.10 $\pm$ 0.09 & 10 $\pm$ 6 \\ 
0.05068 $\pm$ 0.00001 & 13.37 $\pm$ 0.37 & 8 $\pm$ 8 & & 0.29833 $\pm$ 0.00001 & 13.47 $\pm$ 0.04 & 30 $\pm$ 5 \\ 
0.05590 $\pm$ 0.00004 & 13.02 $\pm$ 0.20 & 19 $\pm$ 19 & & 0.30453 $\pm$ 0.00001 & 13.43 $\pm$ 0.09 & 13 $\pm$ 5 \\ 
0.05606 $\pm$ 0.00002 & 13.10 $\pm$ 0.17 & 10 $\pm$ 14 & & 0.30481 $\pm$ 0.00004 & 13.02 $\pm$ 0.16 & 25 $\pm$ 17 \\ 
0.06247 $\pm$ 0.00002 & 13.39 $\pm$ 0.11 & 26 $\pm$ 9 & & 0.30577 $\pm$ 0.00002 & 13.02 $\pm$ 0.21 & 8 $\pm$ 13 \\ 
0.06273 $\pm$ 0.00002 & 13.65 $\pm$ 0.06 & 35 $\pm$ 8 & & 0.30715 $\pm$ 0.00003 & 13.11 $\pm$ 0.14 & 19 $\pm$ 14 \\ 
0.08382 $\pm$ 0.00002 & 13.04 $\pm$ 0.12 & 17 $\pm$ 11 & & 0.30740 $\pm$ 0.00002 & 13.10 $\pm$ 0.12 & 14 $\pm$ 10 \\ 
0.09182 $\pm$ 0.00002 & 12.76 $\pm$ 0.13 & 9 $\pm$ 11 & & 0.31150 $\pm$ 0.00001 & 13.90 $\pm$ 0.03 & 38 $\pm$ 5 \\ 
0.09314 $\pm$ 0.00002 & 12.84 $\pm$ 0.12 & 9 $\pm$ 9 & & 0.33426 $\pm$ 0.00003 & 13.24 $\pm$ 0.12 & 19 $\pm$ 10 \\ 
0.09336 $\pm$ 0.00002 & 12.86 $\pm$ 0.11 & 13 $\pm$ 9 & & 0.33453 $\pm$ 0.00002 & 13.21 $\pm$ 0.38 & 8 $\pm$ 16 \\ 
0.10301 $\pm$ 0.00012 & 13.25 $\pm$ 0.37 & 40 $\pm$ 50 & & 0.35265 $\pm$ 0.00002 & 13.11 $\pm$ 0.08 & 28 $\pm$ 9 \\ 
0.10992 $\pm$ 0.00002 & 13.39 $\pm$ 0.05 & 54 $\pm$ 9 & & 0.35469 $\pm$ 0.00002 & 13.37 $\pm$ 0.05 & 42 $\pm$ 7 \\ 
0.11516 $\pm$ 0.00001 & 13.20 $\pm$ 0.08 & 10 $\pm$ 5 & & 0.36248 $\pm$ 0.00001 & 13.22 $\pm$ 0.10 & 11 $\pm$ 6 \\ 
0.11537 $\pm$ 0.00001 & 13.48 $\pm$ 0.04 & 21 $\pm$ 3 & & 0.36305 $\pm$ 0.00001 & 13.14 $\pm$ 0.18 & 8 $\pm$ 7 \\ 
0.14099 $\pm$ 0.00001 & 13.09 $\pm$ 0.11 & 8 $\pm$ 5 & & 0.36336 $\pm$ 0.00003 & 12.70 $\pm$ 0.22 & 8 $\pm$ 18 \\ 
0.14220 $\pm$ 0.00001 & 13.07 $\pm$ 0.07 & 15 $\pm$ 5 & & 0.36357 $\pm$ 0.00002 & 13.18 $\pm$ 0.09 & 15 $\pm$ 8 \\ 
0.14584 $\pm$ 0.00001 & 13.42 $\pm$ 0.04 & 35 $\pm$ 4 & & 0.36381 $\pm$ 0.00002 & 12.83 $\pm$ 0.17 & 8 $\pm$ 13 \\ 
0.14975 $\pm$ 0.00001 & 13.02 $\pm$ 0.16 & 8 $\pm$ 9 & & 0.37144 $\pm$ 0.00001 & 14.09 $\pm$ 0.02 & 43 $\pm$ 3 \\ 
0.15366 $\pm$ 0.00002 & 12.93 $\pm$ 0.12 & 14 $\pm$ 9 & & 0.37192 $\pm$ 0.00002 & 12.84 $\pm$ 0.16 & 8 $\pm$ 12 \\ 
0.15509 $\pm$ 0.00002 & 13.03 $\pm$ 0.09 & 24 $\pm$ 9 & & 0.37310 $\pm$ 0.00003 & 13.69 $\pm$ 0.07 & 47 $\pm$ 10 \\ 
0.15544 $\pm$ 0.00001 & 13.30 $\pm$ 0.06 & 15 $\pm$ 4 & & 0.37361 $\pm$ 0.00010 & 13.09 $\pm$ 0.24 & 47 $\pm$ 34 \\ 
0.15569 $\pm$ 0.00001 & 13.35 $\pm$ 0.05 & 20 $\pm$ 5 & & 0.37715 $\pm$ 0.00002 & 12.93 $\pm$ 0.09 & 19 $\pm$ 8 \\ 
0.15605 $\pm$ 0.00002 & 13.10 $\pm$ 0.09 & 29 $\pm$ 10 & & 0.39247 $\pm$ 0.00002 & 12.99 $\pm$ 0.08 & 15 $\pm$ 6 \\ 
0.16321 $\pm$ 0.00002 & 13.18 $\pm$ 0.09 & 29 $\pm$ 10 & & 0.40992 $\pm$ 0.00003 & 13.00 $\pm$ 0.15 & 22 $\pm$ 15 \\ 
0.16583 $\pm$ 0.00002 & 13.13 $\pm$ 0.06 & 32 $\pm$ 7 & & 0.41383 $\pm$ 0.00001 & 13.90 $\pm$ 0.03 & 41 $\pm$ 3 \\ 
0.17849 $\pm$ 0.00003 & 13.60 $\pm$ 0.04 & 102 $\pm$ 11 & & 0.41758 $\pm$ 0.00001 & 14.58 $\pm$ 0.06 & 25 $\pm$ 4 \\ 
0.18521 $\pm$ 0.00002 & 12.87 $\pm$ 0.11 & 15 $\pm$ 8 & & 0.41808 $\pm$ 0.00009 & 14.43 $\pm$ 0.23 & 36 $\pm$ 18 \\ 
0.18539 $\pm$ 0.00001 & 12.96 $\pm$ 0.10 & 14 $\pm$ 8 & & 0.41837 $\pm$ 0.00005 & 15.62 $\pm$ 0.23 & 19 $\pm$ 8 \\ 
0.18564 $\pm$ 0.00001 & 13.35 $\pm$ 0.06 & 24 $\pm$ 6 & & 0.41857 $\pm$ 0.00001 & 16.84 $\pm$ 0.05 & 17 $\pm$ 1 \\ 
0.18582 $\pm$ 0.00002 & 12.77 $\pm$ 0.20 & 10 $\pm$ 12 & & 0.41969 $\pm$ 0.00000 & 15.67 $\pm$ 0.05 & 23 $\pm$ 1 \\ 
0.18598 $\pm$ 0.00002 & 12.60 $\pm$ 0.16 & 10 $\pm$ 13 & & 0.42659 $\pm$ 0.00001 & 13.15 $\pm$ 0.07 & 14 $\pm$ 6 \\ 
0.18619 $\pm$ 0.00002 & 12.56 $\pm$ 0.15 & 10 $\pm$ 11 & & 0.42680 $\pm$ 0.00006 & 12.79 $\pm$ 0.45 & 8 $\pm$ 23 \\ 
0.18644 $\pm$ 0.00002 & 12.55 $\pm$ 0.15 & 10 $\pm$ 11 & & 0.42693 $\pm$ 0.00004 & 13.03 $\pm$ 0.26 & 10 $\pm$ 18 \\ 
0.18798 $\pm$ 0.00001 & 13.21 $\pm$ 0.04 & 26 $\pm$ 4 & & 0.43314 $\pm$ 0.00001 & 13.53 $\pm$ 0.04 & 22 $\pm$ 3 \\ 
0.19333 $\pm$ 0.00003 & 12.99 $\pm$ 0.09 & 36 $\pm$ 12 & & 0.43347 $\pm$ 0.00002 & 13.13 $\pm$ 0.08 & 19 $\pm$ 7 \\ 
0.19924 $\pm$ 0.00002 & 13.30 $\pm$ 0.05 & 58 $\pm$ 8 & & 0.43397 $\pm$ 0.00001 & 13.78 $\pm$ 0.03 & 41 $\pm$ 4 \\ 
0.20011 $\pm$ 0.00002 & 12.74 $\pm$ 0.12 & 8 $\pm$ 14 & & 0.44195 $\pm$ 0.00001 & 13.66 $\pm$ 0.03 & 39 $\pm$ 4 \\ 
0.20025 $\pm$ 0.00003 & 12.59 $\pm$ 0.18 & 8 $\pm$ 20 & & 0.45188 $\pm$ 0.00002 & 12.97 $\pm$ 0.08 & 15 $\pm$ 6 \\ 
0.20408 $\pm$ 0.00002 & 12.92 $\pm$ 0.07 & 20 $\pm$ 7 & & 0.47278 $\pm$ 0.00002 & 13.14 $\pm$ 0.12 & 11 $\pm$ 8 \\ 
0.20817 $\pm$ 0.00001 & 13.39 $\pm$ 0.07 & 17 $\pm$ 6 & & 0.47320 $\pm$ 0.00001 & 13.65 $\pm$ 0.05 & 23 $\pm$ 4 \\ 
0.20838 $\pm$ 0.00004 & 12.87 $\pm$ 0.20 & 19 $\pm$ 18 & & 0.47823 $\pm$ 0.00004 & 14.14 $\pm$ 0.05 & 83 $\pm$ 13 \\ 
0.22007 $\pm$ 0.00021 & 12.68 $\pm$ 0.90 & 26 $\pm$ 54 & & 0.72534 $\pm$ 0.00002 & 14.41 $\pm$ 0.05 & 37 $\pm$ 6 \\ 
0.22023 $\pm$ 0.00003 & 13.16 $\pm$ 0.28 & 15 $\pm$ 10 & & 0.76332 $\pm$ 0.00005 & 14.59 $\pm$ 2.61 & 16 $\pm$ 33 \\ 
0.22186 $\pm$ 0.00001 & 13.89 $\pm$ 0.03 & 48 $\pm$ 5 & & 0.76362 $\pm$ 0.00004 & 14.13 $\pm$ 0.25 & 11 $\pm$ 11 \\ 
0.22739 $\pm$ 0.00004 & 12.76 $\pm$ 0.21 & 14 $\pm$ 18 & & 0.83074 $\pm$ 0.00002 & 14.97 $\pm$ 0.04 & 32 $\pm$ 4 \\ 
0.22844 $\pm$ 0.00001 & 14.17 $\pm$ 0.06 & 30 $\pm$ 3 & & 0.83698 $\pm$ 0.00001 & 16.39 $\pm$ 0.03 & 28 $\pm$ 2 \\ 
0.22876 $\pm$ 0.00004 & 12.89 $\pm$ 0.23 & 15 $\pm$ 19 & & 0.83740 $\pm$ 0.00001 & 16.29 $\pm$ 0.03 & 24 $\pm$ 2 \\ 
0.22904 $\pm$ 0.00005 & 13.00 $\pm$ 0.17 & 30 $\pm$ 21 & & 0.83942 $\pm$ 0.00001 & 16.11 $\pm$ 0.03 & 34 $\pm$ 2 \\ 
0.23456 $\pm$ 0.00005 & 12.82 $\pm$ 0.27 & 15 $\pm$ 25 & & \dots & \dots & \dots \\ 

\hline

    \end{tabular}
    
  \end{minipage}
\end{table*}


==> tabs/HI_J1022_body.tex <==

\begin{table*}
\centering
\begin{minipage}{\textwidth}
\caption{\hi~absorption systems in QSO J102218.99+013218.8.}\label{tab:HI_J1022}
\begin{tabular}{@{}cc.ccc.@{}}

\hline                            

$z$ & $\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) & & $z&
$\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) \ 


\hline
-0.00637 $\pm$ 0.00004 & 13.86 $\pm$ 0.13 & 50 $\pm$ 19 & & 0.18013 $\pm$ 0.00002 & 12.99 $\pm$ 0.09 & 17 $\pm$ 8 \\ 
0.00002 $\pm$ 0.00005 & 20.57 $\pm$ 0.02 & 183 $\pm$ 7 & & 0.18039 $\pm$ 0.00001 & 13.17 $\pm$ 0.06 & 24 $\pm$ 6 \\ 
0.03608 $\pm$ 0.00001 & 14.03 $\pm$ 0.08 & 21 $\pm$ 4 & & 0.19674 $\pm$ 0.00010 & 13.32 $\pm$ 0.41 & 28 $\pm$ 26 \\ 
0.03629 $\pm$ 0.00004 & 12.97 $\pm$ 0.20 & 20 $\pm$ 17 & & 0.19688 $\pm$ 0.00003 & 13.22 $\pm$ 0.44 & 10 $\pm$ 16 \\ 
0.04891 $\pm$ 0.00003 & 12.96 $\pm$ 0.21 & 10 $\pm$ 17 & & 0.20902 $\pm$ 0.00002 & 13.17 $\pm$ 0.10 & 13 $\pm$ 8 \\ 
0.05050 $\pm$ 0.00013 & 13.06 $\pm$ 0.62 & 29 $\pm$ 41 & & 0.21171 $\pm$ 0.00003 & 12.76 $\pm$ 0.20 & 10 $\pm$ 20 \\ 
0.05072 $\pm$ 0.00007 & 13.38 $\pm$ 0.30 & 32 $\pm$ 25 & & 0.21392 $\pm$ 0.00003 & 12.87 $\pm$ 0.17 & 10 $\pm$ 15 \\ 
0.05689 $\pm$ 0.00002 & 14.94 $\pm$ 1.73 & 22 $\pm$ 16 & & 0.21518 $\pm$ 0.00006 & 12.87 $\pm$ 0.38 & 10 $\pm$ 34 \\ 
0.05717 $\pm$ 0.00006 & 13.45 $\pm$ 0.22 & 30 $\pm$ 21 & & 0.21573 $\pm$ 0.00006 & 12.88 $\pm$ 0.38 & 10 $\pm$ 33 \\ 
0.05829 $\pm$ 0.00004 & 13.38 $\pm$ 0.13 & 38 $\pm$ 18 & & 0.21712 $\pm$ 0.00008 & 12.90 $\pm$ 0.48 & 10 $\pm$ 46 \\ 
0.05862 $\pm$ 0.00001 & 13.85 $\pm$ 0.17 & 18 $\pm$ 6 & & 0.21728 $\pm$ 0.00010 & 12.82 $\pm$ 0.55 & 10 $\pm$ 55 \\ 
0.07238 $\pm$ 0.00001 & 14.10 $\pm$ 0.04 & 35 $\pm$ 3 & & 0.21926 $\pm$ 0.00001 & 14.87 $\pm$ 0.02 & 29 $\pm$ 1 \\ 
0.08547 $\pm$ 0.00002 & 13.13 $\pm$ 0.16 & 10 $\pm$ 10 & & 0.23231 $\pm$ 0.00001 & 13.75 $\pm$ 0.08 & 18 $\pm$ 4 \\ 
0.08847 $\pm$ 0.00004 & 12.95 $\pm$ 0.21 & 19 $\pm$ 20 & & 0.23257 $\pm$ 0.00001 & 14.26 $\pm$ 2.06 & 10 $\pm$ 10 \\ 
0.08993 $\pm$ 0.00002 & 12.97 $\pm$ 0.17 & 10 $\pm$ 13 & & 0.27861 $\pm$ 0.00002 & 13.17 $\pm$ 0.16 & 10 $\pm$ 9 \\ 
0.09073 $\pm$ 0.00004 & 13.05 $\pm$ 0.17 & 26 $\pm$ 19 & & 0.27900 $\pm$ 0.00002 & 13.71 $\pm$ 0.05 & 34 $\pm$ 6 \\ 
0.09107 $\pm$ 0.00002 & 12.90 $\pm$ 0.18 & 10 $\pm$ 15 & & 0.27943 $\pm$ 0.00001 & 14.06 $\pm$ 0.05 & 26 $\pm$ 4 \\ 
0.09136 $\pm$ 0.00004 & 12.71 $\pm$ 0.24 & 10 $\pm$ 21 & & 0.27983 $\pm$ 0.00006 & 13.29 $\pm$ 0.16 & 46 $\pm$ 24 \\ 
0.09256 $\pm$ 0.00002 & 12.99 $\pm$ 0.16 & 10 $\pm$ 12 & & 0.30151 $\pm$ 0.00003 & 14.16 $\pm$ 0.28 & 29 $\pm$ 13 \\ 
0.09312 $\pm$ 0.00002 & 13.20 $\pm$ 0.10 & 21 $\pm$ 9 & & 0.30342 $\pm$ 0.00001 & 13.75 $\pm$ 0.09 & 19 $\pm$ 5 \\ 
0.11606 $\pm$ 0.00001 & 13.15 $\pm$ 0.13 & 10 $\pm$ 8 & & 0.30370 $\pm$ 0.00002 & 13.45 $\pm$ 0.10 & 18 $\pm$ 8 \\ 
0.11918 $\pm$ 0.00001 & 13.54 $\pm$ 0.05 & 24 $\pm$ 5 & & 0.30668 $\pm$ 0.00001 & 14.10 $\pm$ 0.05 & 24 $\pm$ 2 \\ 
0.12363 $\pm$ 0.00003 & 12.76 $\pm$ 0.22 & 12 $\pm$ 19 & & 0.30876 $\pm$ 0.00002 & 13.30 $\pm$ 0.20 & 10 $\pm$ 9 \\ 
0.12381 $\pm$ 0.00002 & 13.16 $\pm$ 0.18 & 10 $\pm$ 11 & & 0.30898 $\pm$ 0.00001 & 13.64 $\pm$ 0.39 & 10 $\pm$ 7 \\ 
0.12413 $\pm$ 0.00001 & 13.81 $\pm$ 0.05 & 23 $\pm$ 3 & & 0.30954 $\pm$ 0.00002 & 13.45 $\pm$ 0.26 & 10 $\pm$ 8 \\ 
0.13320 $\pm$ 0.00001 & 13.57 $\pm$ 0.23 & 10 $\pm$ 5 & & 0.30973 $\pm$ 0.00002 & 13.27 $\pm$ 0.19 & 10 $\pm$ 10 \\ 
0.13487 $\pm$ 0.00003 & 13.30 $\pm$ 0.09 & 34 $\pm$ 11 & & 0.31432 $\pm$ 0.00002 & 13.14 $\pm$ 0.15 & 13 $\pm$ 11 \\ 
0.13734 $\pm$ 0.00001 & 14.30 $\pm$ 0.05 & 25 $\pm$ 3 & & 0.36086 $\pm$ 0.00002 & 13.20 $\pm$ 0.18 & 10 $\pm$ 10 \\ 
0.14619 $\pm$ 0.00003 & 12.97 $\pm$ 0.20 & 10 $\pm$ 15 & & 0.36108 $\pm$ 0.00006 & 12.71 $\pm$ 0.34 & 10 $\pm$ 28 \\ 
0.14922 $\pm$ 0.00003 & 13.23 $\pm$ 0.19 & 10 $\pm$ 13 & & 0.41031 $\pm$ 0.00001 & 14.67 $\pm$ 0.03 & 28 $\pm$ 1 \\ 
0.14939 $\pm$ 0.00010 & 13.09 $\pm$ 0.63 & 14 $\pm$ 48 & & 0.41886 $\pm$ 0.00004 & 13.72 $\pm$ 0.12 & 22 $\pm$ 9 \\ 
0.16006 $\pm$ 0.00002 & 13.04 $\pm$ 0.13 & 10 $\pm$ 8 & & 0.43259 $\pm$ 0.00002 & 13.41 $\pm$ 0.09 & 21 $\pm$ 7 \\ 
0.16611 $\pm$ 0.00002 & 13.25 $\pm$ 0.07 & 25 $\pm$ 7 & & 0.74259 $\pm$ 0.00001 & 15.68 $\pm$ 0.07 & 14 $\pm$ 1 \\ 
0.17254 $\pm$ 0.00002 & 12.87 $\pm$ 0.13 & 10 $\pm$ 10 & & 0.77966 $\pm$ 0.00003 & 15.25 $\pm$ 0.05 & 52 $\pm$ 7 \\ 
0.17291 $\pm$ 0.00002 & 12.92 $\pm$ 0.12 & 10 $\pm$ 9 & & \dots & \dots & \dots \\ 

\hline

    \end{tabular}
    
  \end{minipage}
\end{table*}


==> tabs/HI_J2218_body.tex <==

\begin{table*}
\centering
\begin{minipage}{\textwidth}
\caption{\hi~absorption systems in QSO J221806.67+005223.6.}\label{tab:HI_J2218}
\begin{tabular}{@{}cc.ccc.@{}}

\hline                            

$z$ & $\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) & & $z&
$\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) \ 


\hline
0.78873 $\pm$ 0.00005 & 14.22 $\pm$ 0.02 & 142 $\pm$ 13 & & 0.99914 $\pm$ 0.00009 & 13.86 $\pm$ 0.04 & 112 $\pm$ 23 \\ 
0.80150 $\pm$ 0.00010 & 14.21 $\pm$ 0.06 & 111 $\pm$ 26 & & 1.01249 $\pm$ 0.00011 & 13.81 $\pm$ 0.06 & 87 $\pm$ 28 \\ 
0.80925 $\pm$ 0.00010 & 14.28 $\pm$ 0.04 & 183 $\pm$ 24 & & 1.01578 $\pm$ 0.00010 & 14.08 $\pm$ 0.04 & 148 $\pm$ 24 \\ 
0.83959 $\pm$ 0.00009 & 14.19 $\pm$ 0.13 & 61 $\pm$ 30 & & 1.04816 $\pm$ 0.00003 & 14.84 $\pm$ 0.08 & 71 $\pm$ 5 \\ 
0.84166 $\pm$ 0.00006 & 15.05 $\pm$ 0.61 & 94 $\pm$ 38 & & 1.05169 $\pm$ 0.00008 & 14.04 $\pm$ 0.04 & 121 $\pm$ 18 \\ 
0.84403 $\pm$ 0.00009 & 14.12 $\pm$ 0.09 & 72 $\pm$ 28 & & 1.08466 $\pm$ 0.00035 & 14.11 $\pm$ 0.14 & 190 $\pm$ 38 \\ 
0.87848 $\pm$ 0.00012 & 15.58 $\pm$ 2.87 & 96 $\pm$ 99 & & 1.09329 $\pm$ 0.00006 & 14.28 $\pm$ 1.64 & 27 $\pm$ 39 \\ 
0.91984 $\pm$ 0.00079 & 13.68 $\pm$ 0.42 & 147 $\pm$ 143 & & 1.09891 $\pm$ 0.00007 & 14.00 $\pm$ 0.35 & 33 $\pm$ 27 \\ 
0.92111 $\pm$ 0.00023 & 13.73 $\pm$ 0.36 & 77 $\pm$ 45 & & 1.13013 $\pm$ 0.00004 & 15.23 $\pm$ 0.56 & 24 $\pm$ 6 \\ 
0.94447 $\pm$ 0.00047 & 14.00 $\pm$ 0.13 & 315 $\pm$ 106 & & 1.21380 $\pm$ 0.00003 & 14.51 $\pm$ 0.30 & 39 $\pm$ 9 \\ 
0.94789 $\pm$ 0.00022 & 14.18 $\pm$ 0.13 & 191 $\pm$ 62 & & 1.21741 $\pm$ 0.00002 & 15.88 $\pm$ 0.59 & 70 $\pm$ 12 \\ 
0.94804 $\pm$ 0.00007 & 14.30 $\pm$ 1.07 & 36 $\pm$ 60 & & \dots & \dots & \dots \\ 

\hline

    \end{tabular}
    
  \end{minipage}
\end{table*}


==> tabs/HI_Q0107A_body.tex <==

\begin{table*}
\centering
\begin{minipage}{\textwidth}
\caption{\hi~absorption systems in QSO Q0107-025A.}\label{tab:HI_Q0107A}
\begin{tabular}{@{}cc.ccc.@{}}

\hline                            

$z$ & $\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) & & $z&
$\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) \ 


\hline
0.00379 $\pm$ 0.00002 & 13.72 $\pm$ 0.04 & 62 $\pm$ 9 & & 0.50173 $\pm$ 0.00002 & 14.36 $\pm$ 0.03 & 46 $\pm$ 3 \\ 
0.00628 $\pm$ 0.00000 & 14.52 $\pm$ 0.03 & 55 $\pm$ 2 & & 0.53568 $\pm$ 0.00001 & 15.30 $\pm$ 0.02 & 60 $\pm$ 4 \\ 
0.04047 $\pm$ 0.00001 & 13.55 $\pm$ 0.03 & 29 $\pm$ 6 & & 0.53644 $\pm$ 0.00001 & 15.91 $\pm$ 0.04 & 38 $\pm$ 2 \\ 
0.04307 $\pm$ 0.00002 & 13.46 $\pm$ 0.11 & 47 $\pm$ 5 & & 0.55752 $\pm$ 0.00001 & 14.91 $\pm$ 0.02 & 45 $\pm$ 2 \\ 
0.05288 $\pm$ 0.00000 & 14.38 $\pm$ 0.05 & 40 $\pm$ 2 & & 0.58037 $\pm$ 0.00007 & 13.95 $\pm$ 0.03 & 208 $\pm$ 24 \\ 
0.05811 $\pm$ 0.00001 & 13.15 $\pm$ 0.07 & 19 $\pm$ 6 & & 0.58648 $\pm$ 0.00014 & 13.46 $\pm$ 0.08 & 114 $\pm$ 63 \\ 
0.06057 $\pm$ 0.00001 & 13.77 $\pm$ 0.04 & 24 $\pm$ 3 & & 0.63392 $\pm$ 0.00009 & 13.91 $\pm$ 0.03 & 251 $\pm$ 29 \\ 
0.06301 $\pm$ 0.00001 & 13.94 $\pm$ 0.02 & 63 $\pm$ 4 & & 0.64025 $\pm$ 0.00002 & 14.22 $\pm$ 0.04 & 40 $\pm$ 6 \\ 
0.07799 $\pm$ 0.00001 & 14.67 $\pm$ 0.21 & 34 $\pm$ 4 & & 0.64365 $\pm$ 0.00006 & 13.62 $\pm$ 0.03 & 85 $\pm$ 20 \\ 
0.08190 $\pm$ 0.00001 & 13.77 $\pm$ 0.05 & 27 $\pm$ 4 & & 0.65808 $\pm$ 0.00015 & 14.09 $\pm$ 0.03 & 491 $\pm$ 46 \\ 
0.09428 $\pm$ 0.00001 & 13.28 $\pm$ 0.06 & 16 $\pm$ 4 & & 0.66372 $\pm$ 0.00012 & 13.70 $\pm$ 0.10 & 116 $\pm$ 40 \\ 
0.10950 $\pm$ 0.00000 & 13.89 $\pm$ 0.04 & 25 $\pm$ 2 & & 0.66635 $\pm$ 0.00012 & 14.12 $\pm$ 0.07 & 285 $\pm$ 68 \\ 
0.11441 $\pm$ 0.00001 & 13.37 $\pm$ 0.07 & 27 $\pm$ 5 & & 0.66901 $\pm$ 0.00017 & 13.58 $\pm$ 0.14 & 121 $\pm$ 52 \\ 
0.11486 $\pm$ 0.00005 & 13.36 $\pm$ 0.09 & 81 $\pm$ 25 & & 0.67482 $\pm$ 0.00019 & 13.74 $\pm$ 0.05 & 389 $\pm$ 64 \\ 
0.11556 $\pm$ 0.00000 & 15.18 $\pm$ 0.14 & 33 $\pm$ 2 & & 0.67931 $\pm$ 0.00008 & 13.91 $\pm$ 0.04 & 117 $\pm$ 28 \\ 
0.12071 $\pm$ 0.00002 & 13.43 $\pm$ 0.05 & 46 $\pm$ 7 & & 0.68985 $\pm$ 0.00004 & 13.79 $\pm$ 0.03 & 65 $\pm$ 20 \\ 
0.13143 $\pm$ 0.00001 & 13.70 $\pm$ 0.03 & 39 $\pm$ 3 & & 0.69448 $\pm$ 0.00008 & 13.69 $\pm$ 2.86 & 18 $\pm$ 126 \\ 
0.16608 $\pm$ 0.00001 & 13.56 $\pm$ 0.03 & 54 $\pm$ 4 & & 0.70193 $\pm$ 0.00012 & 13.25 $\pm$ 0.07 & 107 $\pm$ 45 \\ 
0.17764 $\pm$ 0.00001 & 14.69 $\pm$ 0.04 & 48 $\pm$ 1 & & 0.71267 $\pm$ 0.00005 & 13.48 $\pm$ 0.06 & 37 $\pm$ 19 \\ 
0.19886 $\pm$ 0.00003 & 13.26 $\pm$ 0.05 & 61 $\pm$ 10 & & 0.71867 $\pm$ 0.00004 & 14.23 $\pm$ 0.02 & 193 $\pm$ 12 \\ 
0.20244 $\pm$ 0.00000 & 14.01 $\pm$ 0.01 & 52 $\pm$ 2 & & 0.71889 $\pm$ 0.00000 & 15.66 $\pm$ 0.03 & 23 $\pm$ 1 \\ 
0.22569 $\pm$ 0.00000 & 13.64 $\pm$ 0.05 & 15 $\pm$ 2 & & 0.72808 $\pm$ 0.00002 & 14.22 $\pm$ 0.05 & 24 $\pm$ 2 \\ 
0.22619 $\pm$ 0.00000 & 14.18 $\pm$ 0.04 & 22 $\pm$ 1 & & 0.72883 $\pm$ 0.00002 & 14.42 $\pm$ 0.04 & 40 $\pm$ 2 \\ 
0.22718 $\pm$ 0.00000 & 15.62 $\pm$ 0.03 & 42 $\pm$ 1 & & 0.73794 $\pm$ 0.00051 & 13.25 $\pm$ 0.21 & 188 $\pm$ 103 \\ 
0.23382 $\pm$ 0.00002 & 14.27 $\pm$ 0.02 & 60 $\pm$ 4 & & 0.76554 $\pm$ 0.00115 & 13.67 $\pm$ 0.22 & 618 $\pm$ 374 \\ 
0.23746 $\pm$ 0.00001 & 13.99 $\pm$ 0.07 & 21 $\pm$ 2 & & 0.78646 $\pm$ 0.00002 & 14.30 $\pm$ 0.02 & 90 $\pm$ 7 \\ 
0.23770 $\pm$ 0.00003 & 13.92 $\pm$ 0.07 & 48 $\pm$ 7 & & 0.79937 $\pm$ 0.00025 & 13.75 $\pm$ 0.06 & 341 $\pm$ 72 \\ 
0.24956 $\pm$ 0.00001 & 13.19 $\pm$ 0.10 & 7 $\pm$ 5 & & 0.80720 $\pm$ 0.00009 & 13.44 $\pm$ 0.05 & 96 $\pm$ 32 \\ 
0.26111 $\pm$ 0.00004 & 13.61 $\pm$ 0.06 & 92 $\pm$ 17 & & 0.81112 $\pm$ 0.00023 & 13.18 $\pm$ 0.11 & 147 $\pm$ 72 \\ 
0.26165 $\pm$ 0.00000 & 14.30 $\pm$ 0.03 & 31 $\pm$ 1 & & 0.82175 $\pm$ 0.00038 & 13.61 $\pm$ 0.08 & 441 $\pm$ 105 \\ 
0.26285 $\pm$ 0.00005 & 13.54 $\pm$ 0.13 & 54 $\pm$ 8 & & 0.83441 $\pm$ 0.00063 & 13.30 $\pm$ 0.15 & 248 $\pm$ 27 \\ 
0.29478 $\pm$ 0.00001 & 13.77 $\pm$ 0.03 & 29 $\pm$ 3 & & 0.84327 $\pm$ 0.00006 & 13.64 $\pm$ 0.03 & 100 $\pm$ 21 \\ 
0.33276 $\pm$ 0.00002 & 13.69 $\pm$ 0.06 & 45 $\pm$ 7 & & 0.84782 $\pm$ 0.00002 & 14.03 $\pm$ 0.22 & 34 $\pm$ 16 \\ 
0.35516 $\pm$ 0.00002 & 13.16 $\pm$ 0.07 & 24 $\pm$ 7 & & 0.86880 $\pm$ 0.00003 & 13.81 $\pm$ 0.14 & 34 $\pm$ 19 \\ 
0.35688 $\pm$ 0.00001 & 13.44 $\pm$ 0.04 & 19 $\pm$ 3 & & 0.87634 $\pm$ 0.00001 & 15.96 $\pm$ 0.06 & 19 $\pm$ 1 \\ 
0.38470 $\pm$ 0.00000 & 14.74 $\pm$ 0.01 & 51 $\pm$ 1 & & 0.87660 $\pm$ 0.00010 & 14.97 $\pm$ 0.24 & 36 $\pm$ 7 \\ 
0.38854 $\pm$ 0.00003 & 13.26 $\pm$ 0.06 & 48 $\pm$ 10 & & 0.88964 $\pm$ 0.00002 & 13.89 $\pm$ 0.11 & 24 $\pm$ 6 \\ 
0.39908 $\pm$ 0.00004 & 13.51 $\pm$ 0.08 & 54 $\pm$ 13 & & 0.89900 $\pm$ 0.00234 & 14.20 $\pm$ 0.38 & 31 $\pm$ 50 \\ 
0.39950 $\pm$ 0.00001 & 14.29 $\pm$ 0.03 & 26 $\pm$ 1 & & 0.90643 $\pm$ 0.00007 & 14.88 $\pm$ 0.09 & 30 $\pm$ 0 \\ 
0.41657 $\pm$ 0.00001 & 13.80 $\pm$ 0.03 & 46 $\pm$ 4 & & 0.92637 $\pm$ 0.00005 & 14.24 $\pm$ 0.02 & 124 $\pm$ 17 \\ 
0.42968 $\pm$ 0.00001 & 14.31 $\pm$ 0.02 & 76 $\pm$ 3 & & 0.94970 $\pm$ 0.00012 & 13.64 $\pm$ 0.05 & 78 $\pm$ 59 \\ 
0.48792 $\pm$ 0.00017 & 13.92 $\pm$ 0.07 & 240 $\pm$ 72 & & 0.95673 $\pm$ 0.00003 & 14.68 $\pm$ 0.06 & 30 $\pm$ 0 \\ 
0.50048 $\pm$ 0.00001 & 14.25 $\pm$ 0.04 & 34 $\pm$ 2 & & 0.96531 $\pm$ 0.00004 & 15.16 $\pm$ 0.26 & 14 $\pm$ 1 \\ 

\hline

    \end{tabular}
    
  \end{minipage}
\end{table*}


==> tabs/HI_Q0107B_body.tex <==

\begin{table*}
\centering
\begin{minipage}{\textwidth}
\caption{\hi~absorption systems in QSO Q0107-025B.}\label{tab:HI_Q0107B}
\begin{tabular}{@{}cc.ccc.@{}}

\hline                            

$z$ & $\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) & & $z&
$\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) \ 


\hline
0.00634 $\pm$ 0.00000 & 14.30 $\pm$ 0.08 & 31 $\pm$ 3 & & 0.39916 $\pm$ 0.00001 & 15.26 $\pm$ 0.12 & 51 $\pm$ 3 \\ 
0.01337 $\pm$ 0.00001 & 13.35 $\pm$ 0.05 & 22 $\pm$ 5 & & 0.41236 $\pm$ 0.00001 & 13.91 $\pm$ 0.03 & 26 $\pm$ 3 \\ 
0.04175 $\pm$ 0.00001 & 13.51 $\pm$ 0.04 & 42 $\pm$ 6 & & 0.42768 $\pm$ 0.00003 & 13.40 $\pm$ 0.07 & 38 $\pm$ 9 \\ 
0.05319 $\pm$ 0.00001 & 13.64 $\pm$ 0.04 & 33 $\pm$ 5 & & 0.43428 $\pm$ 0.00001 & 13.75 $\pm$ 0.03 & 35 $\pm$ 4 \\ 
0.06068 $\pm$ 0.00001 & 13.32 $\pm$ 0.06 & 28 $\pm$ 6 & & 0.43612 $\pm$ 0.00002 & 13.74 $\pm$ 0.04 & 62 $\pm$ 7 \\ 
0.06312 $\pm$ 0.00001 & 13.47 $\pm$ 0.04 & 24 $\pm$ 3 & & 0.46746 $\pm$ 0.00001 & 14.04 $\pm$ 0.03 & 44 $\pm$ 3 \\ 
0.10963 $\pm$ 0.00001 & 13.26 $\pm$ 0.06 & 26 $\pm$ 6 & & 0.49937 $\pm$ 0.00001 & 15.00 $\pm$ 0.08 & 30 $\pm$ 3 \\ 
0.11530 $\pm$ 0.00000 & 13.51 $\pm$ 0.04 & 32 $\pm$ 4 & & 0.49954 $\pm$ 0.00007 & 14.72 $\pm$ 0.17 & 57 $\pm$ 7 \\ 
0.11571 $\pm$ 0.00000 & 14.53 $\pm$ 0.06 & 32 $\pm$ 1 & & 0.51226 $\pm$ 0.00010 & 13.64 $\pm$ 0.54 & 22 $\pm$ 58 \\ 
0.12031 $\pm$ 0.00001 & 13.51 $\pm$ 0.04 & 22 $\pm$ 3 & & 0.51707 $\pm$ 0.00001 & 14.65 $\pm$ 0.02 & 44 $\pm$ 3 \\ 
0.12073 $\pm$ 0.00001 & 13.82 $\pm$ 0.02 & 48 $\pm$ 3 & & 0.52383 $\pm$ 0.00005 & 14.08 $\pm$ 0.29 & 44 $\pm$ 33 \\ 
0.13638 $\pm$ 0.00000 & 13.85 $\pm$ 0.03 & 26 $\pm$ 2 & & 0.53536 $\pm$ 0.00001 & 15.18 $\pm$ 0.04 & 29 $\pm$ 2 \\ 
0.15465 $\pm$ 0.00002 & 15.89 $\pm$ 0.59 & 22 $\pm$ 2 & & 0.55558 $\pm$ 0.00012 & 13.68 $\pm$ 1.64 & 26 $\pm$ 171 \\ 
0.15513 $\pm$ 0.00023 & 13.39 $\pm$ 0.27 & 64 $\pm$ 16 & & 0.57853 $\pm$ 0.00008 & 13.76 $\pm$ 0.11 & 33 $\pm$ 23 \\ 
0.20020 $\pm$ 0.00000 & 15.62 $\pm$ 0.00 & 26 $\pm$ 0 & & 0.62198 $\pm$ 0.00012 & 13.81 $\pm$ 2.29 & 26 $\pm$ 163 \\ 
0.20252 $\pm$ 0.00000 & 14.94 $\pm$ 0.02 & 43 $\pm$ 1 & & 0.64271 $\pm$ 0.00291 & 13.72 $\pm$ 1.47 & 184 $\pm$ 94 \\ 
0.20303 $\pm$ 0.00000 & 14.76 $\pm$ 0.03 & 26 $\pm$ 1 & & 0.66027 $\pm$ 0.00041 & 13.86 $\pm$ 2.60 & 13 $\pm$ 62 \\ 
0.21192 $\pm$ 0.00001 & 13.28 $\pm$ 0.04 & 26 $\pm$ 4 & & 0.71364 $\pm$ 0.00002 & 14.30 $\pm$ 0.05 & 24 $\pm$ 4 \\ 
0.22669 $\pm$ 0.00000 & 14.97 $\pm$ 0.04 & 28 $\pm$ 1 & & 0.71797 $\pm$ 0.00006 & 15.29 $\pm$ 0.05 & 47 $\pm$ 11 \\ 
0.22714 $\pm$ 0.00001 & 13.92 $\pm$ 0.02 & 49 $\pm$ 4 & & 0.71840 $\pm$ 0.00011 & 14.82 $\pm$ 0.14 & 26 $\pm$ 25 \\ 
0.25416 $\pm$ 0.00003 & 13.36 $\pm$ 0.06 & 56 $\pm$ 11 & & 0.78724 $\pm$ 0.00008 & 14.08 $\pm$ 0.03 & 139 $\pm$ 11 \\ 
0.25809 $\pm$ 0.00001 & 13.28 $\pm$ 0.04 & 31 $\pm$ 4 & & 0.79769 $\pm$ 0.00014 & 13.65 $\pm$ 0.07 & 128 $\pm$ 47 \\ 
0.26107 $\pm$ 0.00000 & 14.75 $\pm$ 0.01 & 61 $\pm$ 1 & & 0.80943 $\pm$ 0.00007 & 15.21 $\pm$ 0.14 & 29 $\pm$ 8 \\ 
0.29456 $\pm$ 0.00001 & 13.81 $\pm$ 0.03 & 38 $\pm$ 4 & & 0.83185 $\pm$ 0.00004 & 14.26 $\pm$ 0.63 & 17 $\pm$ 7 \\ 
0.31421 $\pm$ 0.00005 & 13.74 $\pm$ 0.09 & 56 $\pm$ 12 & & 0.84776 $\pm$ 0.00023 & 13.57 $\pm$ 0.08 & 170 $\pm$ 47 \\ 
0.31453 $\pm$ 0.00001 & 13.65 $\pm$ 0.10 & 24 $\pm$ 5 & & 0.87597 $\pm$ 0.00014 & 15.29 $\pm$ 0.12 & 24 $\pm$ 15 \\ 
0.32176 $\pm$ 0.00001 & 13.75 $\pm$ 1.83 & 6 $\pm$ 7 & & 0.87673 $\pm$ 0.00027 & 14.62 $\pm$ 0.32 & 13 $\pm$ 15 \\ 
0.33333 $\pm$ 0.00001 & 13.75 $\pm$ 0.04 & 33 $\pm$ 4 & & 0.88990 $\pm$ 0.00011 & 13.96 $\pm$ 0.41 & 14 $\pm$ 7 \\ 
0.38312 $\pm$ 0.00001 & 13.32 $\pm$ 0.08 & 12 $\pm$ 3 & & 0.90724 $\pm$ 0.00003 & 14.61 $\pm$ 0.08 & 50 $\pm$ 3 \\ 
0.39911 $\pm$ 0.00000 & 16.84 $\pm$ 0.02 & 20 $\pm$ 1 & & 0.92625 $\pm$ 0.00012 & 13.99 $\pm$ 2.75 & 20 $\pm$ 90 \\ 

\hline

    \end{tabular}
    
  \end{minipage}
\end{table*}


==> tabs/HI_Q0107C_body.tex <==

\begin{table*}
\centering
\begin{minipage}{\textwidth}
\caption{\hi~absorption systems in QSO Q0107-0232 .}\label{tab:HI_Q0107C}
\begin{tabular}{@{}cc.ccc.@{}}

\hline                            

$z$ & $\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) & & $z&
$\log{N_{
m HI}({
m cm}^{-2})}$ & $b_{
m HI}$ (\kms) \ 


\hline
0.19895 $\pm$ 0.00001 & 14.73 $\pm$ 0.11 & 52 $\pm$ 5 & & 0.42513 $\pm$ 0.00001 & 13.93 $\pm$ 0.04 & 37 $\pm$ 5 \\ 
0.20335 $\pm$ 0.00002 & 14.79 $\pm$ 0.15 & 42 $\pm$ 6 & & 0.42831 $\pm$ 0.00000 & 16.01 $\pm$ 0.18 & 35 $\pm$ 2 \\ 
0.22710 $\pm$ 0.00000 & 14.00 $\pm$ 0.00 & 50 $\pm$ 0 & & 0.43637 $\pm$ 0.00001 & 13.76 $\pm$ 0.06 & 23 $\pm$ 10 \\ 
0.24472 $\pm$ 0.00000 & 14.00 $\pm$ 0.00 & 50 $\pm$ 0 & & 0.44184 $\pm$ 0.00006 & 14.26 $\pm$ 0.03 & 208 $\pm$ 17 \\ 
0.26140 $\pm$ 0.00002 & 14.02 $\pm$ 0.05 & 43 $\pm$ 6 & & 0.44459 $\pm$ 0.00004 & 13.70 $\pm$ 0.05 & 80 $\pm$ 13 \\ 
0.26653 $\pm$ 0.00000 & 14.53 $\pm$ 0.07 & 49 $\pm$ 4 & & 0.48712 $\pm$ 0.00022 & 14.08 $\pm$ 0.06 & 384 $\pm$ 76 \\ 
0.26837 $\pm$ 0.00001 & 13.28 $\pm$ 0.14 & 9 $\pm$ 5 & & 0.49973 $\pm$ 0.00014 & 14.03 $\pm$ 0.32 & 61 $\pm$ 95 \\ 
0.26864 $\pm$ 0.00001 & 13.80 $\pm$ 0.07 & 16 $\pm$ 2 & & 0.53459 $\pm$ 0.00001 & 16.11 $\pm$ 0.10 & 25 $\pm$ 2 \\ 
0.28163 $\pm$ 0.00003 & 13.23 $\pm$ 0.11 & 40 $\pm$ 14 & & 0.55739 $\pm$ 0.00000 & 19.49 $\pm$ 0.04 & 50 $\pm$ 0 \\ 
0.29449 $\pm$ 0.00003 & 13.86 $\pm$ 0.08 & 28 $\pm$ 7 & & 0.57854 $\pm$ 0.00002 & 14.83 $\pm$ 0.32 & 17 $\pm$ 8 \\ 
0.30885 $\pm$ 0.00002 & 13.46 $\pm$ 0.05 & 34 $\pm$ 8 & & 0.57875 $\pm$ 0.00010 & 15.02 $\pm$ 0.22 & 42 $\pm$ 13 \\ 
0.33116 $\pm$ 0.00002 & 13.74 $\pm$ 0.06 & 40 $\pm$ 7 & & 0.62200 $\pm$ 0.00002 & 14.49 $\pm$ 0.04 & 40 $\pm$ 4 \\ 
0.35050 $\pm$ 0.00019 & 13.12 $\pm$ 0.45 & 43 $\pm$ 49 & & 0.64871 $\pm$ 0.00001 & 15.53 $\pm$ 0.09 & 27 $\pm$ 2 \\ 
0.35565 $\pm$ 0.00004 & 13.32 $\pm$ 0.08 & 47 $\pm$ 13 & & 0.64974 $\pm$ 0.00032 & 13.81 $\pm$ 0.10 & 123 $\pm$ 33 \\ 
0.35798 $\pm$ 0.00001 & 13.53 $\pm$ 0.05 & 27 $\pm$ 5 & & 0.68366 $\pm$ 0.00008 & 14.22 $\pm$ 0.02 & 327 $\pm$ 25 \\ 
0.36540 $\pm$ 0.00001 & 13.58 $\pm$ 0.05 & 30 $\pm$ 5 & & 0.68979 $\pm$ 0.00002 & 14.87 $\pm$ 0.04 & 66 $\pm$ 3 \\ 
0.37587 $\pm$ 0.00003 & 13.50 $\pm$ 0.07 & 41 $\pm$ 9 & & 0.69004 $\pm$ 0.00002 & 14.30 $\pm$ 0.12 & 14 $\pm$ 6 \\ 
0.38022 $\pm$ 0.00001 & 13.15 $\pm$ 0.07 & 13 $\pm$ 4 & & 0.69993 $\pm$ 0.00038 & 13.21 $\pm$ 0.20 & 51 $\pm$ 0 \\ 
0.38099 $\pm$ 0.00001 & 13.49 $\pm$ 0.09 & 11 $\pm$ 3 & & 0.70111 $\pm$ 0.00019 & 13.43 $\pm$ 0.13 & 50 $\pm$ 0 \\ 
0.38138 $\pm$ 0.00000 & 13.95 $\pm$ 0.30 & 11 $\pm$ 3 & & 0.71121 $\pm$ 0.00003 & 14.06 $\pm$ 0.07 & 28 $\pm$ 4 \\ 
0.40166 $\pm$ 0.00003 & 13.69 $\pm$ 0.76 & 8 $\pm$ 9 & & 0.71735 $\pm$ 0.00001 & 14.89 $\pm$ 0.03 & 29 $\pm$ 1 \\ 
0.41666 $\pm$ 0.00112 & 13.69 $\pm$ 0.98 & 152 $\pm$ 173 & & 0.71806 $\pm$ 0.00003 & 14.37 $\pm$ 0.10 & 20 $\pm$ 5 \\ 
0.41752 $\pm$ 0.00038 & 13.94 $\pm$ 0.54 & 131 $\pm$ 45 & & 0.71831 $\pm$ 0.00001 & 15.06 $\pm$ 0.05 & 15 $\pm$ 2 \\ 
0.42381 $\pm$ 0.00003 & 13.55 $\pm$ 0.06 & 46 $\pm$ 9 & & 0.71874 $\pm$ 0.00001 & 14.64 $\pm$ 0.04 & 27 $\pm$ 2 \\ 
0.42458 $\pm$ 0.00001 & 14.03 $\pm$ 0.04 & 36 $\pm$ 4 & & 0.73886 $\pm$ 0.00009 & 13.39 $\pm$ 0.06 & 30 $\pm$ 0 \\ 

\hline

    \end{tabular}
    
  \end{minipage}
\end{table*}


==> tabs/HI_gal_summary.tex <==
\begin{table}
  \begin{minipage}{0.45\textwidth}
    \centering
    \caption{Summary of the \hi absorption systems and galaxie sused in
      the cross-correlation analysis.}\label{tab:HI_gal_summary}
    \begin{tabular}{@{}lcccccc@{}}
    \hline
     Label     & \multicolumn{3}{c}{\hi systems}&\multicolumn{3}{c}{Galaxies} \\
               & \SF    &   \nSF    &  Total    &   \strong     &  \weak   & Total \\
    \hline
    `a'        
    
    \end{tabular}
  \end{minipage}
\end{table}


==> tabs/gal_GDDS_summary.tex <==
%\begin{table*}
%  \centering
%  %\begin{minipage}{180mm}
%  \caption{Summary of our galaxy sample}\label{tab:gal_survey_summary}
%  \begin{tabular}{@{}llrrrrr@{}}
%    \hline
%    Confidence & &\multicolumn{2}{c}{Galaxies} & Stars & AGN & Unknown \\
%    \cmidrule(r){3-4}
%               & &Star-forming & Non-star-forming &    &     &   \\
%    \hline
%    Secure  &(`a')  & 1336     & 298              &451 & 2   &0  \\
%    Possible &(`b') & 441      & 68               & 42 & 20  &0  \\
%    No idea  &(`c') & 0        & 0                & 0  & 0   &893\\
%    Undefined &(`n')& \multicolumn{2}{c}{31}      & 0  & 0   &0\\
%    \hline
%    \end{tabular}
%    
%  %\end{minipage}
%\end{table*}

\begin{table}
  \begin{minipage}{0.5\textwidth}
    \centering
    \caption{Summary of the GDDS survey used in this paper.}\label{tab:gal_GDDS_summary}
    \begin{tabular}{@{}lcccc@{}}
    \hline
               & Secure & Possible & No idea & Total\\
               & (`a')  & (`b')    & (`c')   & \\
    \hline
    Galaxies   & 41  & 12       & 0          & 53\\
    \ \ \SF    & 32  & 11       & 0       & 43\\
    \ \ \nSF   & 9   & 1        & 0       & 10\\
    Stars      & 1   & 0        & 0       & 1 \\
    AGN        & 1   & 0        & 0       & 1\\
    Unknown    & 0   & 0        & 5       & 5\\
    \hline
    \end{tabular}
  \end{minipage}
\end{table}



==> tabs/gal_VVDS_summary.tex <==
%\begin{table*}
%  \centering
%  %\begin{minipage}{180mm}
%  \caption{Summary of our galaxy sample}\label{tab:gal_survey_summary}
%  \begin{tabular}{@{}llrrrrr@{}}
%    \hline
%    Confidence & &\multicolumn{2}{c}{Galaxies} & Stars & AGN & Unknown \\
%    \cmidrule(r){3-4}
%               & &Star-forming & Non-star-forming &    &     &   \\
%    \hline
%    Secure  &(`a')  & 1336     & 298              &451 & 2   &0  \\
%    Possible &(`b') & 441      & 68               & 42 & 20  &0  \\
%    No idea  &(`c') & 0        & 0                & 0  & 0   &893\\
%    Undefined &(`n')& \multicolumn{2}{c}{31}      & 0  & 0   &0\\
%    \hline
%    \end{tabular}
%    
%  %\end{minipage}
%\end{table*}

\begin{table}
  \begin{minipage}{0.5\textwidth}
    \centering
    \caption{Summary of the VVDS survey used in this
      paper.}\label{tab:gal_VVDS_summary}
    \begin{tabular}{@{}lcccc@{}}
    \hline
               & Secure & Possible & No idea & Total\\
               & (`a')  & (`b')    & (`c')   & \\
    \hline
    Galaxies   & 9458   & 7903     & 0       & 17361\\
    Stars      & 1      & 2        & 0       & 3 \\
    AGN        & 138    & 131      & 0       & 269\\
    Unknown    & 0      & 0        & 8394    & 8394\\
    \hline
    \end{tabular}
  \end{minipage}
\end{table}



==> tabs/gals_J1005_body.tex <==
\begin{table*}
\centering
\begin{minipage}{\textwidth}
\caption{Spectroscopic catalog of objects in the J1005 field.}\label{tab:gals_J1005}
\begin{tabular}{@{}cccccccc@{}}
\hline                            
R.A. (J2000) & Dec. (J2000) & $z$ & $z$ label& Spec. Type & $R$     &  CLASS\_STAR & Instrument \\ 

(degrees)    & (degrees)    &     &          &            &   (mag) &              &            \\ 

\hline

151.2010830 & 1.4927170 & 0.00101 & a & star	 & 18.579 $\pm$ 0.002 & 0.98 & VIMOS\\ 
151.2026460 & 1.6136780 & 1.20432 & b & SF	 & 22.886 $\pm$ 0.053 & 0.66 & VIMOS\\ 
151.2027620 & 1.4385080 & 0.12836 & b & SF	 & 22.170 $\pm$ 0.027 & 0.15 & VIMOS\\ 
151.2041830 & 1.4458021 & 0.97918 & b & non-SF	 & \dots & \dots & VIMOS\\ 
151.2041830 & 1.4487940 & \dots & c & none	 & 22.614 $\pm$ 0.037 & 0.70 & VIMOS\\ 
151.2046920 & 1.6611220 & \dots & c & none	 & 21.741 $\pm$ 0.028 & 0.00 & VIMOS\\ 
151.2050670 & 1.6475640 & -0.00011 & a & star	 & 21.298 $\pm$ 0.014 & 0.98 & VIMOS\\ 
151.2059290 & 1.5797750 & 0.50199 & a & SF	 & 21.653 $\pm$ 0.020 & 0.57 & VIMOS\\ 
151.2065420 & 1.4616330 & \dots & c & none	 & 21.372 $\pm$ 0.012 & 0.98 & VIMOS\\ 
151.2073670 & 1.5225190 & 0.37406 & a & SF	 & 21.908 $\pm$ 0.022 & 0.90 & VIMOS\\ 
151.2074540 & 1.4413060 & \dots & c & none	 & 20.681 $\pm$ 0.013 & 0.01 & VIMOS\\ 
151.2078630 & 1.5926220 & 0.67556 & a & SF	 & 22.494 $\pm$ 0.050 & 0.00 & VIMOS\\ 
151.2078630 & 1.6566250 & 0.61715 & a & SF	 & 21.617 $\pm$ 0.025 & 0.02 & VIMOS\\ 
151.2080670 & 1.5194170 & 0.37583 & a & SF	 & 21.596 $\pm$ 0.017 & 0.07 & VIMOS\\ 
151.2082380 & 1.6196750 & \dots & c & none	 & 20.765 $\pm$ 0.009 & 0.98 & VIMOS\\ 
151.2087580 & 1.6543750 & 0.41405 & a & SF	 & 20.712 $\pm$ 0.011 & 0.02 & VIMOS\\ 
151.2089790 & 1.6019140 & -0.00034 & a & star	 & 21.905 $\pm$ 0.025 & 0.96 & VIMOS\\ 
151.2089880 & 1.6083250 & 0.18328 & a & SF	 & 19.755 $\pm$ 0.006 & 0.03 & VIMOS\\ 
151.2101170 & 1.4302190 & 0.00069 & a & star	 & 20.752 $\pm$ 0.008 & 0.98 & VIMOS\\ 
151.2103880 & 1.4997830 & 0.61862 & a & SF	 & 21.792 $\pm$ 0.019 & 0.52 & VIMOS\\ 
151.2109420 & 1.4809360 & 0.33694 & b & SF	 & 19.818 $\pm$ 0.007 & 0.03 & VIMOS\\ 
151.2113670 & 1.5629190 & 0.42171 & a & SF	 & \dots & \dots & VIMOS\\ 
151.2150080 & 1.4586720 & -0.00022 & a & star	 & 22.152 $\pm$ 0.024 & 0.95 & VIMOS\\ 
151.2162420 & 1.6629030 & 0.43493 & a & non-SF	 & 19.598 $\pm$ 0.006 & 0.03 & VIMOS\\ 
151.2168960 & 1.4660310 & 0.00038 & b & star	 & 21.815 $\pm$ 0.021 & 0.96 & VIMOS\\ 
151.2176500 & 1.6055970 & 0.30463 & b & SF	 & 20.243 $\pm$ 0.008 & 0.03 & VIMOS\\ 
151.2176620 & 1.5107060 & 0.26676 & a & SF	 & 21.070 $\pm$ 0.013 & 0.03 & VIMOS\\ 
151.2185960 & 1.6270190 & 0.36074 & a & non-SF	 & 20.222 $\pm$ 0.007 & 0.98 & VIMOS\\ 
151.2191250 & 1.4710440 & 0.27843 & a & SF	 & 21.228 $\pm$ 0.017 & 0.10 & VIMOS\\ 
151.2191670 & 1.4690420 & 0.84391 & a & SF	 & 20.982 $\pm$ 0.011 & 0.79 & VIMOS\\ 
151.2200750 & 1.5978030 & -0.00058 & b & star	 & 19.450 $\pm$ 0.004 & 0.98 & VIMOS\\ 
151.2204790 & 1.5964030 & 0.37994 & a & SF	 & 20.745 $\pm$ 0.012 & 0.37 & VIMOS\\ 
151.2218250 & 1.6312110 & 0.34083 & a & SF	 & 21.820 $\pm$ 0.024 & 0.44 & VIMOS\\ 
151.2221170 & 1.6682970 & 0.43573 & a & non-SF	 & 19.022 $\pm$ 0.005 & 0.03 & VIMOS\\ 
151.2254120 & 1.6245890 & 0.59725 & a & SF	 & 21.904 $\pm$ 0.026 & 0.15 & VIMOS\\ 
151.2270330 & 1.5736720 & 0.17725 & a & SF	 & 20.043 $\pm$ 0.007 & 0.04 & VIMOS\\ 
151.2279330 & 1.5093390 & \dots & c & none	 & 22.682 $\pm$ 0.052 & 0.00 & VIMOS\\ 
151.2280170 & 1.6455110 & 0.43082 & a & SF	 & 21.841 $\pm$ 0.025 & 0.15 & VIMOS\\ 
151.2285250 & 1.4762780 & 0.41303 & a & SF	 & 20.854 $\pm$ 0.009 & 0.97 & VIMOS\\ 
151.2288210 & 1.4897830 & 1.24987 & b & AGN	 & 21.292 $\pm$ 0.012 & 0.98 & VIMOS\\ 
151.2303210 & 1.6742750 & 0.46584 & a & SF	 & 20.774 $\pm$ 0.013 & 0.02 & VIMOS\\ 
151.2313880 & 1.4788860 & \dots & c & none	 & 20.009 $\pm$ 0.005 & 0.98 & VIMOS\\ 
151.2343960 & 1.5014280 & 0.09836 & a & SF	 & 21.062 $\pm$ 0.011 & 0.98 & VIMOS\\ 
151.2343960 & 1.5027300 & 0.95041 & b & SF	 & 22.765 $\pm$ 0.044 & 0.26 & VIMOS\\ 
151.2351670 & 1.6039030 & 0.69146 & a & SF	 & 21.842 $\pm$ 0.026 & 0.01 & VIMOS\\ 
151.2362130 & 1.4434170 & 0.42208 & a & non-SF	 & 20.645 $\pm$ 0.009 & 0.93 & VIMOS\\ 
151.2384870 & 1.5838470 & 0.22287 & a & SF	 & 19.486 $\pm$ 0.004 & 0.05 & VIMOS\\ 
151.2396210 & 1.4354830 & 0.22180 & a & SF	 & 20.103 $\pm$ 0.009 & 0.02 & VIMOS\\ 
151.2401120 & 1.4519560 & \dots & c & none	 & 21.992 $\pm$ 0.021 & 0.96 & VIMOS\\ 
151.2407000 & 1.4924269 & \dots & c & none	 & \dots & \dots & VIMOS\\ 

\hline

    \end{tabular}
    
  \end{minipage}
\end{table*}


==> tabs/gals_J1022_body.tex <==

\begin{table*}
\centering
\begin{minipage}{\textwidth}
\caption{Spectroscopic catalog of objects in the J1022 field.}\label{tab:gals_J1022}
\begin{tabular}{@{}cccccccc@{}}
\hline                            
R.A. (J2000) & Dec. (J2000) & $z$ & $z$ label& Spec. Type & $R$     &  CLASS\_STAR & Instrument \\ 

(degrees)    & (degrees)    &     &          &            &   (mag) &              &            \\ 

\hline

155.3771500 & 1.3965470 & 0.85070 & a & SF	 & 21.136 $\pm$ 0.021 & 0.00 & VIMOS\\ 
155.3828420 & 1.4153000 & 1.14834 & b & SF	 & 22.998 $\pm$ 0.058 & 0.00 & VIMOS\\ 
155.3842040 & 1.4004060 & 0.00003 & a & star	 & 20.402 $\pm$ 0.007 & 0.98 & VIMOS\\ 
155.3858330 & 1.4708640 & 0.60021 & a & non-SF	 & 21.040 $\pm$ 0.014 & 0.02 & VIMOS\\ 
155.3870580 & 1.4858810 & 0.58565 & b & non-SF	 & \dots & \dots & VIMOS\\ 
155.3883210 & 1.4655670 & 0.60243 & a & non-SF	 & 21.432 $\pm$ 0.018 & 0.13 & VIMOS\\ 
155.3885710 & 1.4063670 & -0.00010 & a & star	 & 21.471 $\pm$ 0.014 & 0.98 & VIMOS\\ 
155.3888170 & 1.4522470 & 0.58591 & a & SF	 & 21.532 $\pm$ 0.015 & 0.42 & VIMOS\\ 
155.3896710 & 1.4872670 & 0.58497 & a & SF	 & \dots & \dots & VIMOS\\ 
155.3903120 & 1.4598140 & 0.38725 & a & non-SF	 & 21.559 $\pm$ 0.017 & 0.19 & VIMOS\\ 
155.3913670 & 1.4424000 & 0.27934 & a & SF	 & 21.605 $\pm$ 0.024 & 0.03 & VIMOS\\ 
155.3931330 & 1.3758110 & 0.32796 & a & SF	 & 22.366 $\pm$ 0.034 & 0.05 & VIMOS\\ 
155.3931670 & 1.3805470 & 0.50953 & a & SF	 & 21.316 $\pm$ 0.013 & 0.14 & VIMOS\\ 
155.3943500 & 1.4399780 & \dots & c & none	 & 21.246 $\pm$ 0.011 & 0.98 & VIMOS\\ 
155.3949630 & 1.4466420 & 0.83557 & a & AGN	 & 20.403 $\pm$ 0.007 & 0.98 & VIMOS\\ 
155.3952500 & 1.4580890 & 0.54344 & a & SF	 & 22.233 $\pm$ 0.030 & 0.01 & VIMOS\\ 
155.3959040 & 1.4101640 & 0.37917 & a & SF	 & 21.457 $\pm$ 0.016 & 0.02 & VIMOS\\ 
155.3968500 & 1.4737060 & 0.38864 & a & non-SF	 & 20.405 $\pm$ 0.008 & 0.04 & VIMOS\\ 
155.3989620 & 1.3915000 & 0.38217 & a & SF	 & 20.134 $\pm$ 0.009 & 0.02 & VIMOS\\ 
155.4010880 & 1.4329530 & 1.18020 & a & SF	 & 21.996 $\pm$ 0.027 & 0.17 & VIMOS\\ 
155.4040420 & 1.4208640 & 0.00012 & a & star	 & 19.672 $\pm$ 0.004 & 0.98 & VIMOS\\ 
155.4057870 & 1.4616420 & 0.43151 & b & non-SF	 & 21.392 $\pm$ 0.015 & 0.40 & VIMOS\\ 
155.4096830 & 1.4803280 & 0.33866 & a & SF	 & 21.712 $\pm$ 0.029 & 0.00 & VIMOS\\ 
155.4099330 & 1.3864440 & 0.53787 & a & SF	 & 21.252 $\pm$ 0.013 & 0.63 & VIMOS\\ 
155.4147290 & 1.4225140 & 0.27044 & a & SF	 & 21.930 $\pm$ 0.021 & 0.96 & VIMOS\\ 
155.4175460 & 1.4826584 & \dots & c & none	 & 20.196 $\pm$ 0.010 & 0.02 & VIMOS\\ 
155.4175460 & 1.4830580 & 0.69187 & a & SF	 & 20.196 $\pm$ 0.010 & 0.02 & VIMOS\\ 
155.4212210 & 1.4134690 & 0.54900 & a & SF	 & 20.532 $\pm$ 0.008 & 0.03 & VIMOS\\ 
155.4218420 & 1.4537690 & 0.74263 & b & non-SF	 & 21.849 $\pm$ 0.031 & 0.00 & VIMOS\\ 
155.4220420 & 1.5014190 & 0.71312 & a & SF	 & 21.264 $\pm$ 0.021 & 0.00 & VIMOS\\ 
155.4223330 & 1.4788440 & -0.00011 & a & star	 & 20.495 $\pm$ 0.010 & 0.15 & VIMOS\\ 
155.4223880 & 1.5088310 & 0.27742 & a & SF	 & \dots & \dots & VIMOS\\ 
155.4224710 & 1.4606890 & 0.66903 & a & SF	 & 21.985 $\pm$ 0.034 & 0.00 & VIMOS\\ 
155.4229710 & 1.4999440 & 0.00005 & a & star	 & 20.846 $\pm$ 0.011 & 0.07 & VIMOS\\ 
155.4230290 & 1.6471830 & 0.00015 & a & star	 & 21.786 $\pm$ 0.017 & 0.98 & VIMOS\\ 
155.4230710 & 1.4494220 & 0.97206 & b & AGN	 & 20.782 $\pm$ 0.009 & 0.88 & VIMOS\\ 
155.4231830 & 1.4244750 & 0.00025 & a & star	 & 19.849 $\pm$ 0.005 & 0.94 & VIMOS\\ 
155.4237750 & 1.4325287 & \dots & c & none	 & \dots & \dots & VIMOS\\ 
155.4237750 & 1.4348330 & 0.37862 & a & SF	 & 22.407 $\pm$ 0.034 & 0.04 & VIMOS\\ 
155.4242080 & 1.5954920 & 0.27933 & b & SF	 & 21.173 $\pm$ 0.021 & 0.01 & VIMOS\\ 
155.4246250 & 1.6511140 & \dots & c & none	 & 21.974 $\pm$ 0.019 & 0.97 & VIMOS\\ 
155.4247960 & 1.5718440 & 0.38384 & a & non-SF	 & 19.492 $\pm$ 0.005 & 0.03 & VIMOS\\ 
155.4248790 & 1.6306220 & 0.26039 & a & SF	 & 22.779 $\pm$ 0.037 & 0.14 & VIMOS\\ 
155.4248830 & 1.5827420 & 0.37303 & a & SF	 & 21.984 $\pm$ 0.025 & 0.01 & VIMOS\\ 
155.4250080 & 1.5785440 & 0.22107 & a & SF	 & 20.848 $\pm$ 0.010 & 0.09 & VIMOS\\ 
155.4251540 & 1.4555170 & 0.18725 & a & SF	 & 20.168 $\pm$ 0.006 & 0.77 & VIMOS\\ 
155.4251830 & 1.5968580 & 0.37088 & b & SF	 & 21.465 $\pm$ 0.019 & 0.00 & VIMOS\\ 
155.4253870 & 1.4045500 & -0.00036 & a & star	 & 21.099 $\pm$ 0.010 & 0.98 & VIMOS\\ 
155.4261670 & 1.5851220 & 0.28037 & a & SF	 & 22.498 $\pm$ 0.030 & 0.78 & VIMOS\\ 
155.4285830 & 1.4029360 & \dots & c & none	 & 21.407 $\pm$ 0.017 & 0.89 & VIMOS\\ 

\hline

    \end{tabular}
    
  \end{minipage}
\end{table*}


==> tabs/gals_J2218_body.tex <==

\begin{table*}
\centering
\begin{minipage}{\textwidth}
\caption{Spectroscopic catalog of objects in the J2218 field.}\label{tab:gals_J2218}
\begin{tabular}{@{}cccccccc@{}}
\hline                            
R.A. (J2000) & Dec. (J2000) & $z$ & $z$ label& Spec. Type & $R$     &  CLASS\_STAR & Instrument \\ 

(degrees)    & (degrees)    &     &          &            &   (mag) &              &            \\ 

\hline

334.3341960 & 0.8822500 & \dots & c & none	 & 22.270 $\pm$ 0.058 & 0.76 & VIMOS\\ 
334.3342670 & 0.8709560 & 0.71389 & a & SF	 & 22.094 $\pm$ 0.064 & 0.06 & VIMOS\\ 
334.3353210 & 0.7628110 & -0.00073 & a & star	 & 21.057 $\pm$ 0.024 & 0.95 & VIMOS\\ 
334.3353920 & 0.9552640 & -0.00059 & a & star	 & 19.970 $\pm$ 0.009 & 0.98 & VIMOS\\ 
334.3354000 & 0.8771310 & -0.00008 & a & star	 & 20.748 $\pm$ 0.017 & 0.98 & VIMOS\\ 
334.3354000 & 0.8781607 & \dots & c & none	 & 20.748 $\pm$ 0.017 & 0.98 & VIMOS\\ 
334.3355330 & 0.8996690 & 0.27697 & a & SF	 & 19.592 $\pm$ 0.011 & 0.02 & VIMOS\\ 
334.3377580 & 0.9407390 & -0.00082 & a & star	 & 20.665 $\pm$ 0.016 & 0.98 & VIMOS\\ 
334.3380540 & 0.7537890 & 0.42663 & a & non-SF	 & 19.790 $\pm$ 0.012 & 0.06 & VIMOS\\ 
334.3384040 & 0.8902330 & -0.00028 & a & star	 & 20.091 $\pm$ 0.010 & 0.98 & VIMOS\\ 
334.3387210 & 0.8685580 & -0.00018 & a & star	 & 22.428 $\pm$ 0.062 & 0.73 & VIMOS\\ 
334.3423750 & 0.8596390 & 0.00004 & a & star	 & 21.184 $\pm$ 0.023 & 0.97 & VIMOS\\ 
334.3426830 & 0.9539360 & 0.35516 & a & SF	 & 19.843 $\pm$ 0.013 & 0.02 & VIMOS\\ 
334.3432920 & 0.8046030 & \dots & c & none	 & 21.940 $\pm$ 0.046 & 0.88 & VIMOS\\ 
334.3447040 & 0.8077670 & 0.56340 & b & SF	 & 21.638 $\pm$ 0.039 & 0.45 & VIMOS\\ 
334.3449750 & 0.8119170 & -0.00062 & a & star	 & 20.938 $\pm$ 0.018 & 0.98 & VIMOS\\ 
334.3449750 & 0.8142394 & \dots & c & none	 & 21.652 $\pm$ 0.044 & 0.16 & VIMOS\\ 
334.3452120 & 0.8023190 & 0.27795 & b & non-SF	 & 20.783 $\pm$ 0.020 & 0.24 & VIMOS\\ 
334.3463920 & 0.9478530 & \dots & c & none	 & 21.481 $\pm$ 0.037 & 0.16 & VIMOS\\ 
334.3467460 & 0.7237310 & \dots & c & none	 & 21.130 $\pm$ 0.035 & 0.00 & VIMOS\\ 
334.3467880 & 0.7062280 & \dots & c & none	 & 21.245 $\pm$ 0.025 & 0.97 & VIMOS\\ 
334.3480790 & 0.8669330 & \dots & c & none	 & 22.229 $\pm$ 0.067 & 0.09 & VIMOS\\ 
334.3481130 & 0.7282940 & \dots & c & none	 & 21.042 $\pm$ 0.029 & 0.01 & VIMOS\\ 
334.3483670 & 0.9086940 & \dots & c & none	 & 20.457 $\pm$ 0.013 & 0.98 & VIMOS\\ 
334.3489920 & 0.7443720 & \dots & c & none	 & 20.694 $\pm$ 0.018 & 0.98 & VIMOS\\ 
334.3495710 & 0.7150110 & 2.67752 & b & AGN	 & 20.321 $\pm$ 0.013 & 0.98 & VIMOS\\ 
334.3500420 & 0.7344670 & 0.51024 & a & SF	 & 21.104 $\pm$ 0.032 & 0.01 & VIMOS\\ 
334.3500420 & 0.7373342 & \dots & c & none	 & \dots & \dots & VIMOS\\ 
334.3502880 & 0.7793440 & \dots & c & none	 & 20.718 $\pm$ 0.024 & 0.01 & VIMOS\\ 
334.3506170 & 0.9300920 & \dots & c & none	 & 21.479 $\pm$ 0.046 & 0.00 & VIMOS\\ 
334.3511580 & 0.8944060 & 0.51967 & a & non-SF	 & 20.512 $\pm$ 0.022 & 0.04 & VIMOS\\ 
334.3517000 & 0.7695060 & 0.25191 & a & SF	 & 21.662 $\pm$ 0.049 & 0.01 & VIMOS\\ 
334.3518000 & 0.7991670 & 0.00008 & a & star	 & 22.586 $\pm$ 0.065 & 0.73 & VIMOS\\ 
334.3521170 & 0.7812030 & -0.00097 & a & star	 & 18.718 $\pm$ 0.005 & 0.90 & VIMOS\\ 
334.3530250 & 0.9675690 & -0.00105 & a & star	 & 20.355 $\pm$ 0.012 & 0.98 & VIMOS\\ 
334.3531670 & 0.7180360 & \dots & c & none	 & 20.451 $\pm$ 0.016 & 0.42 & VIMOS\\ 
334.3541710 & 0.9166720 & \dots & c & none	 & 19.978 $\pm$ 0.016 & 0.01 & VIMOS\\ 
334.3547250 & 0.8168470 & -0.00047 & a & star	 & 19.150 $\pm$ 0.006 & 0.98 & VIMOS\\ 
334.3548170 & 0.8544640 & \dots & c & none	 & 20.005 $\pm$ 0.010 & 0.98 & VIMOS\\ 
334.3549080 & 0.7828860 & 0.44863 & b & non-SF	 & 21.154 $\pm$ 0.028 & 0.34 & VIMOS\\ 
334.3550580 & 0.7480530 & \dots & c & none	 & 20.750 $\pm$ 0.017 & 0.97 & VIMOS\\ 
334.3558790 & 0.9048810 & \dots & c & none	 & 20.172 $\pm$ 0.011 & 0.98 & VIMOS\\ 
334.3561960 & 0.7588958 & -0.00024 & a & star	 & \dots & \dots & VIMOS\\ 
334.3561960 & 0.7601640 & \dots & c & none	 & 20.694 $\pm$ 0.019 & 0.98 & VIMOS\\ 
334.3564330 & 0.8924420 & 0.00036 & a & star	 & 20.692 $\pm$ 0.015 & 0.98 & VIMOS\\ 
334.3567040 & 0.7414530 & 0.44818 & a & non-SF	 & 20.306 $\pm$ 0.020 & 0.06 & VIMOS\\ 
334.3578620 & 0.7935890 & \dots & c & none	 & 20.379 $\pm$ 0.012 & 0.98 & VIMOS\\ 
334.3600710 & 0.7222830 & 0.36505 & a & SF	 & 20.269 $\pm$ 0.018 & 0.02 & VIMOS\\ 
334.3605880 & 0.9377500 & 0.00060 & a & star	 & 19.993 $\pm$ 0.009 & 0.98 & VIMOS\\ 
334.3607120 & 0.9353610 & 0.33050 & a & SF	 & 20.336 $\pm$ 0.020 & 0.01 & VIMOS\\ 

\hline

    \end{tabular}
    
  \end{minipage}
\end{table*}


==> tabs/gals_Q0107_body.tex <==

\begin{table*}
\centering
\begin{minipage}{\textwidth}
\caption{Spectroscopic catalog of objects in the Q0107 field.}\label{tab:gals_Q0107}
\begin{tabular}{@{}cccccccc@{}}
\hline                            
R.A. (J2000) & Dec. (J2000) & $z$ & $z$ label& Spec. Type & $R$     &  CLASS\_STAR & Instrument \\ 

(degrees)    & (degrees)    &     &          &            &   (mag) &              &            \\ 

\hline

17.3801061 & -2.4595306 & \dots & c & none	 & 22.044 $\pm$ 0.020 & 0.89 & VIMOS\\ 
17.3802944 & -2.4484262 & \dots & c & none	 & 21.582 $\pm$ 0.013 & 0.91 & VIMOS\\ 
17.3806726 & -2.3963086 & \dots & c & none	 & 22.862 $\pm$ 0.027 & 0.85 & VIMOS\\ 
17.3809226 & -2.2929955 & \dots & c & none	 & 22.758 $\pm$ 0.059 & 0.01 & VIMOS\\ 
17.3814706 & -2.4545652 & \dots & c & none	 & 20.598 $\pm$ 0.007 & 0.03 & VIMOS\\ 
17.3815274 & -2.2840227 & 0.82064 & a & SF	 & 22.625 $\pm$ 0.029 & 0.22 & VIMOS\\ 
17.3838253 & -2.3076722 & \dots & c & none	 & 22.847 $\pm$ 0.050 & 0.87 & VIMOS\\ 
17.3838360 & -2.3124420 & 0.20695 & a & SF	 & 21.495 $\pm$ 0.013 & 0.91 & VIMOS\\ 
17.3843259 & -2.4291244 & 0.57581 & a & SF	 & 21.854 $\pm$ 0.018 & 0.98 & VIMOS\\ 
17.3845944 & -2.3804886 & 0.56579 & a & SF	 & 21.460 $\pm$ 0.013 & 0.11 & VIMOS\\ 
17.3859288 & -2.4250594 & \dots & c & none	 & 21.882 $\pm$ 0.033 & 0.72 & VIMOS\\ 
17.3866085 & -2.2721099 & 0.19078 & a & non-SF	 & 18.479 $\pm$ 0.002 & 0.62 & VIMOS\\ 
17.3867188 & -2.4348304 & 0.26042 & a & SF	 & 22.247 $\pm$ 0.041 & 0.04 & VIMOS\\ 
17.3876921 & -2.3904844 & 0.18978 & a & non-SF	 & 18.921 $\pm$ 0.002 & 0.04 & VIMOS\\ 
17.3889915 & -2.3834838 & 0.42979 & a & non-SF	 & 19.573 $\pm$ 0.005 & 0.04 & VIMOS\\ 
17.3894789 & -2.4635309 & \dots & c & none	 & 22.781 $\pm$ 0.058 & 0.15 & VIMOS\\ 
17.3894843 & -2.2802917 & \dots & c & none	 & 22.397 $\pm$ 0.024 & 0.12 & VIMOS\\ 
17.3917423 & -2.2377874 & 0.87501 & b & SF	 & 21.917 $\pm$ 0.020 & 0.06 & VIMOS\\ 
17.3923751 & -2.3238664 & 0.32278 & a & SF	 & 19.355 $\pm$ 0.003 & 0.03 & VIMOS\\ 
17.3934644 & -2.2690468 & 0.56778 & b & SF	 & 22.005 $\pm$ 0.018 & 0.03 & VIMOS\\ 
17.3937199 & -2.2618792 & \dots & c & none	 & 23.222 $\pm$ 0.039 & 0.92 & VIMOS\\ 
17.3938225 & -2.2635220 & 0.12353 & a & SF	 & 20.759 $\pm$ 0.008 & 0.03 & VIMOS\\ 
17.3942498 & -2.3293894 & 0.18578 & a & SF	 & 20.602 $\pm$ 0.006 & 0.03 & VIMOS\\ 
17.3953368 & -2.2225204 & 0.43185 & b & SF	 & 21.519 $\pm$ 0.014 & 0.34 & VIMOS\\ 
17.3954821 & -2.4672036 & 0.43178 & a & SF	 & 21.508 $\pm$ 0.011 & 0.57 & VIMOS\\ 
17.3958049 & -2.3202095 & \dots & c & none	 & 22.844 $\pm$ 0.040 & 0.92 & VIMOS\\ 
17.3968905 & -2.3267592 & \dots & c & none	 & 22.776 $\pm$ 0.046 & 0.10 & VIMOS\\ 
17.3993609 & -2.4447712 & \dots & c & none	 & 21.030 $\pm$ 0.011 & 0.03 & VIMOS\\ 
17.4012395 & -2.2517755 & \dots & c & none	 & 22.862 $\pm$ 0.039 & 0.02 & VIMOS\\ 
17.4016882 & -2.4186022 & \dots & c & none	 & 22.953 $\pm$ 0.035 & 0.05 & VIMOS\\ 
17.4023821 & -2.3679135 & 0.72143 & b & SF	 & 22.919 $\pm$ 0.054 & 0.76 & VIMOS\\ 
17.4025886 & -2.2430918 & 0.56978 & a & SF	 & 22.662 $\pm$ 0.026 & 0.79 & VIMOS\\ 
17.4032523 & -2.2593518 & 0.00000 & b & star	 & 20.685 $\pm$ 0.007 & 0.03 & VIMOS\\ 
17.4033054 & -2.2753482 & 0.75478 & a & SF	 & 21.843 $\pm$ 0.017 & 0.03 & VIMOS\\ 
17.4037058 & -2.2555941 & \dots & c & none	 & 19.752 $\pm$ 0.007 & 0.03 & VIMOS\\ 
17.4056201 & -2.2284788 & \dots & c & none	 & 21.715 $\pm$ 0.013 & 0.25 & VIMOS\\ 
17.4062088 & -2.3933847 & 0.75639 & a & SF	 & 22.671 $\pm$ 0.037 & 0.77 & VIMOS\\ 
17.4064744 & -2.4400682 & 0.00000 & a & star	 & 18.785 $\pm$ 0.001 & 0.98 & VIMOS\\ 
17.4067003 & -2.3012956 & 0.57778 & b & SF	 & 21.372 $\pm$ 0.015 & 0.02 & VIMOS\\ 
17.4080018 & -2.2457734 & 0.57099 & a & SF	 & 20.935 $\pm$ 0.009 & 0.87 & VIMOS\\ 
17.4089544 & -2.2958733 & 0.46930 & a & non-SF	 & 21.614 $\pm$ 0.011 & 0.98 & VIMOS\\ 
17.4093632 & -2.4077866 & 0.51250 & b & SF	 & 21.929 $\pm$ 0.018 & 0.03 & VIMOS\\ 
17.4096565 & -2.2987822 & 0.43184 & b & SF	 & 21.904 $\pm$ 0.014 & 0.73 & VIMOS\\ 
17.4102754 & -2.4147429 & 0.07678 & a & SF	 & 17.722 $\pm$ 0.001 & 0.03 & VIMOS\\ 
17.4115807 & -2.2871535 & 0.00000 & a & star	 & 20.310 $\pm$ 0.004 & 0.98 & VIMOS\\ 
17.4134077 & -2.2197607 & 0.00000 & a & star	 & 21.057 $\pm$ 0.006 & 0.98 & VIMOS\\ 
17.4146583 & -2.4028245 & \dots & c & none	 & 22.323 $\pm$ 0.024 & 0.04 & VIMOS\\ 
17.4147056 & -2.2399490 & 0.57001 & a & SF	 & 21.512 $\pm$ 0.014 & 0.06 & VIMOS\\ 
17.4178072 & -2.4729537 & 0.00000 & a & star	 & 19.767 $\pm$ 0.003 & 0.98 & VIMOS\\ 
17.4178425 & -2.4715606 & \dots & c & none	 & 22.889 $\pm$ 0.051 & 0.16 & VIMOS\\ 

\hline

    \end{tabular}
    
  \end{minipage}
\end{table*}


==> tabs/spectral_indices.tex <==
\begin{table}
  \centering
  %\begin{minipage}{180mm}
    \caption{Definition of our spectral indices bands}\label{tab:samples:spectral_indices}
    \begin{tabular}{@{}lccc@{}}
      \hline
      
      Index    &  Blue side band & Central band & Red side band \\
               &  (\AA)          &  (\AA)       & (\AA) \\
      \hline
      \dfour   &  3750--3950     & \dots        & 4050--4250\\
      \ha      &  6460--6530     & 6530--6610   & 6610--6680\\
      \hb      &  4760--4830     & 4830--4900   & 5030--5100\\
      \hc      &  4200--4270     & 4320--4360   & 4360--4430\\
      \hd      &  4010--4080     & 4085--4120   & 4120--4190\\
      \oii     &  3645--3715     & 3715--3740   & 3740--3810\\
      \oiii    &  4760--4830     & 4990--5030   & 5030--5100\\
      \sii     &  6625--6695     & 6695--6760   & 6760--6830\\
      \hline

    \end{tabular}
    
  %\end{minipage}
\end{table}


==> tabs/xi_T_fits.tex <==
\begin{table}
  \begin{minipage}{0.45\textwidth}
    \centering
    \caption{Real-space correlation function fits (assuming power law
      of the form presented in
      \Cref{eq:rscf}).\tablenotemark{a}}\label{tab:xi_T_fits}
    \begin{tabular}{@{}lrrr@{}}
      \hline 
      \multicolumn{1}{c}{Sample} & \multicolumn{1}{c}{$\xi_{\rm ag}(r)$} &\multicolumn{1}{c}{$\xi_{\rm gg}(r)$} & \multicolumn{1}{c}{$\xi_{\rm aa}(r)$}\\
      \hline
      Full Sample &   2.3 $\pm$  0.8 &  5.7 $\pm$  0.7 &  2.1 $\pm$  0.3\\
      \ \ `Strong'--\SF  &   8.3 $\pm$  2.3 &  6.1 $\pm$  0.6 &  7.5 $\pm$  2.4\\
      \ \ `Strong'--\nSF & 10.3 $\pm$  5.5 & 12.6 $\pm$  3.2 &  7.5 $\pm$  2.4\\
      \ \ `Weak'--\SF    &   0.9 $\pm$  0.6 &  6.1 $\pm$  0.6 &  1.9 $\pm$  0.4 \\
      \ \ `Weak--\nSF    &   0.6 $\pm$  0.4 & 12.6 $\pm$  3.2 &  1.9 $\pm$  0.4 \\
      
      \hline                                     
    \end{tabular}
  \end{minipage}
  \begin{minipage}{0.45\textwidth}
    $^{\rm a}$ Note that peaks are not necessarly at the smallest scale
    bins (see Figures \ref{fig:xi_all} to \ref{fig:xi_ab_wk}).\\
  \end{minipage}
\end{table}


==> tabs/xi_params2.tex <==
\begin{table*}
  \begin{minipage}{0.7\textwidth}
    \centering
    \caption{Real-space correlation function parameter assuming power
      law of the form presented in \Cref{eq:rscf} with fixed $\gamma$}.\label{tab:xi_params2}
    \begin{tabular}{@{}lccccccccccc@{}}
      \hline 
               & \multicolumn{2}{c}{$\xi_{\rm ag}(r)$} &&\multicolumn{2}{c}{$\xi_{\rm gg}(r)$} && \multicolumn{2}{c}{$\xi_{\rm aa}(r)$}\\ 
      \cline{2-4} \cline{6-8}\cline{10-12}
          & $r_0$ & $r_0$  &$r_0$  & & $r_0$  &$r_0$   &$r_0$  & &$r_0$   &$r_0$  & $r_0$ \\
         
          & ($\gamma=1.5$) & $(\gamma=1.6$) & (\gamma=1.7)& & $(\gamma=1.5)$ & $(\gamma=1.6)$ & $(\gamma=1.7)$& & $(\gamma=1.5)$ & $(\gamma=1.6)$ & $(\gamma=1.7)$\\
         
      \hline
      Full Sample        &   1.6 $\pm$  0.2  & 1.5 $\pm$ 0.1   &         &  3.7 $\pm$  0.1 &  1.7 $\pm$  0.1   && 0.0 $\pm$  0.7& 1.0 $\pm$  0.3\\
      \ \ `Strong'--\SF  &   3.8 $\pm$  0.2  & 1.7 $\pm$ 0.1   &         &  3.9 $\pm$  0.1 &  1.6 $\pm$  0.1   && 0.9 $\pm$  0.7& 1.0 $\pm$  0.2\\
      \ \ `Strong'--\nSF &   4.0 $\pm$  0.3  & 1.7 $\pm$ 0.1   &         &  6.2 $\pm$  0.2 &  1.6 $\pm$  0.1   && 0.9 $\pm$  0.7& 1.0 $\pm$  0.2\\
        \ \ `Weak'--\SF  &   0.3 $\pm$  0.4  & 1.1 $\pm$ 0.3   &         &  3.9 $\pm$  0.1 &  1.6 $\pm$  0.1   && 0.4 $\pm$  0.1& 1.1 $\pm$  0.1\\
       \ \ `Weak--\nSF   &   0.0 $\pm$  0.8  & 1.0 $\pm$ 1.4   &         &  6.2 $\pm$  0.2 &  1.6 $\pm$  0.1   && 0.4 $\pm$  0.1& 1.1 $\pm$  0.1\\
       
       \hline                                     
    \end{tabular}
    \end{minipage}
  \end{table*}

